The Yoneda Reduction of Polymorphic Types (Extended Version)

In this paper we explore a family of type isomorphisms in System F whose validity corresponds, semantically, to some form of the Yoneda isomorphism from category theory. These isomorphisms hold under theories of equivalence stronger than beta-eta-equivalence, like those induced by parametricity and dinaturality. We show that the Yoneda type isomorphisms yield a rewriting over types, that we call Yoneda reduction, which can be used to eliminate quantifiers from a polymorphic type, replacing them with a combination of monomorphic type constructors. We establish some sufficient conditions under which quantifiers can be fully eliminated from a polymorphic type, and we show some application of these conditions to count the inhabitants of a type and to compute program equivalence in some fragments of System F.

==> appProofs.tex <==
% !TEX root = YonedaTryAgain.tex



\kappaz*
\begin{proof}%[Proof of Lemma. \ref{lemma:kappa}.]
If $\kappa(\bb E)=\infty$ the claim is trivial.
If $\kappa(\bb E)=1$, then by Lemma \ref{lemma:solvable}, $\kappa(\bb E')\leq 1=\kappa(\bb E)$.

%$\kappa(\bb E)=0$, then $\bb E$ has no  path, which implies that it has no modular edge. Since $\bb E$ is solvable, the only possibility is that for all bound variable $\bb X$, either $\cc X$ or $\mm X$ never occurs. This property is stable under reduction, since a reduction step cannot introduce new labels except for $\bullet$. We deduce that also $\bb E'$ has no modular edge, and thus no path, whence $\kappa(\bb E')=1$. 



Suppose now $\kappa(\bb E)=0$. We must show that there is no cyclic alternate path in $\bb E'$, on the assumption that there is no cyclic path in $\bb E$. Suppose $\bb E'$ is obtained by a reduction as the one in Fig. \ref{fig:11}. 
As in the proof of Lemma \ref{lemma:solvable}, for any node $\alpha$ of $\bb E'$, let $g(\alpha)$ be the unique node in $\bb E$ 
 $\alpha$ ``comes from''.
%Let us define a mapping $g$ from the nodes of $\bb E'$ without label $\bullet$, to the nodes of $\bb E$ as follows:
%if $\alpha$ is a node of $\bb E'$ occurring within either $\bb E_{l}$ or $\cc F$ different from the node replaced by $\cc X\theta$, then $g(\alpha)$ is the same node in in $\bb E$; if $\alpha$ is a node occurring in one of the copies of $\cc{\mathsf D}_{ji}[\cc X\mapsto \bullet]$, or one of the nodes with label $\vec Z_{j}$, then $g(\alpha)$ is the corresponding node in the unique copy of $\cc{\mathsf D}_{ji}[\cc X]$ in $\bb E$. 
We will show that any alternating path from $\gamma_{1}$ to $ \gamma_{n}$ in $\bb E'$ induces an alternate path from $g(\gamma_{1})$ to  $g(\gamma_{n})$ in $\bb E$. From this fact it immediately follows that $\kappa(\bb E')\leq 0$, since any cyclic path in $\bb E'$ would induce a cyclic path in $\bb E$, against the assumption that $\kappa(\bb E)= 0$.

First observe that if $\delta: Y^{c}$ is a modular node in $\bb E'$, then $g(\delta):g( Y)^{c}$ is a modular node in $\bb E$. In fact one can check that:
	\begin{itemize}
	\item if $g(\delta):g(Y)^{ c}$ is the head of the sub-tree of $\bb E$ rooted in $\bb r_{g(Y)}$, then also $\delta$ is the head of the sub-tree of $\bb E'$ rooted in $\bb r_{Y}$ (it suffices to check for the cases $\bb r_{g(Y)}\preceq \bb r_{X}$ and $\bb r_{g(X)}\prec \bb r_{X}$);
	\item if $d(g(\delta), \bb r_{g(Y)})>2$, then $d(\delta, \bb r_{Y})>2$ (again, one has to check the cases $\bb r_{g(Y)}\preceq \bb r_{X}$ and $\bb r_{g(X)}\prec \bb r_{X}$);
	
 	\item if $g(\delta): g(Y)^{ c}$ has a parallel node $\beta: g(Y)^{ c}$, then also $\delta:Y^{ c}$ has a parallel node $\beta':Y^{ c}$ with $g(\beta')=\beta$.
	\end{itemize}
From this it follows that if $(\gamma: Y^{c})\step (\delta: Y^{\OV c})$ is a down-move in $\bb E'$; then $(g(\gamma): g(Y)^{c})\step (g(\delta):g( Y)^{\OV c})$ is a down-move in $\bb E$. 
Moreover, if $(\gamma: Y^{c})\step (\delta: Z^{d})$ is an up-move in $\bb E'$, then two possibilities arise:

	\begin{itemize}
	\item  $\gamma: Y^{c}$ is a modular node occurring either in some of the $\FFun{\cc X\mapsto \cc\bullet}{\cc{\mathsf D}_{jk}}$ or of the $\FFun{\cc X\theta}{\mm{\mathsf F}_{l}}$, and $\delta: Z^{d}$ is a terminal node in the same sub-tree. Then $g(\gamma)$ is a modular node
 occurring either in some copy of $\FFun{\cc X}{\cc{\mathsf D}_{jk}}$ or in $\FFun{\cc X}{\mm{\mathsf F}_{l}}$
 and $g(\delta)$ is a terminal node in the same sub-tree, so we conclude that $g(\gamma)\step g(\delta)$ is an up-move in  $\bb E$.



	\item $\gamma: Y^{c}$ is a modular node occurring in some copy of $\FFun{\cc X\theta}{\mm{\mathsf F}_{l}}$, and $\delta: Z^{d}$ is a terminal node in the sub-tree $\FFun{\cc X\mapsto \cc\bullet}{\cc{\mathsf D}_{jk}}$ which is on top of $\FFun{\cc X\theta}{\mm{\mathsf F}_{l}}$. Then $g(\gamma)$ is modular in $\bb E$ and by construction there exists a terminal node $\alpha:\cc X$ in $\FFun{\cc X\theta}{\mm{\mathsf F}_{l}}$, a modular node $\beta: \mm X$ in $\FFun{\cc X}{\cc{\mathsf D}_{jk}}$, so that there is an alternate path $g(\gamma)\step \alpha\step \beta\step g(\delta)$ in $\bb E$, as illustrated in Fig. \ref{fig:cycle}. 	
	
%	 the same sub-tree. Then $g(\gamma)$ is a modular node
% occurring either in some copy of $\FFun{\cc X\mapsto \cc\bullet}{D_{jk}}$ or in $\FFun{\cc X\theta}{\mm{\mathsf F}_{l}}$
% and $g(\delta)$ is a terminal node in the same sub-tree, so we conclude that $g(\gamma)\step g(\delta)$ is a up-move in  $\bb E$.
%
%
%	
%	 $\gamma: Y^{c}$ is a modular node occurring in either some $\mm E_{l}$ or in $\cc F$ and $\delta: Z^{d}$ is a terminal node in $\cc{\mathsf D}_{ji}$. Then $g(\gamma)$ is a modular node in $\mm E_{l}[\cc X]$ or $\cc F[\cc X]$ in $\bb E$ (for the same reason of the previous points)  
%and $g(\delta)$ is a terminal node in $\cc{\mathsf D}_{ji}[\cc X]$, and there is a modular edge $(\alpha:\cc X,\beta:\mm X)$ such that $\alpha$ is terminal in $\mm E_{l}[\cc X]$ (or $\cc F[\cc X]$), $\beta$ is the head of a $\bb X$-module in which $\cc{\mathsf D}_{ji}[\cc X]$ occurs and there is a path $g(\gamma)\step \alpha \step \beta \step g(\delta)$ in $\bb E$ (see Fig. \ref{fig:cycle}).
	 \end{itemize}
	 
We conclude that if $\alpha_{0}\dots \alpha_{2n}$ is an alternate path in $\bb E'$, then we can find an alternate path 
$g(\alpha_{0})g(\alpha_{1})\dots g(\alpha_{2})g(\alpha_{3})\dots g(\alpha_{2n-2})g(\alpha_{2n-1})\dots g(\alpha_{2n})$ in $\bb E$.
	 
A similar argument can be developed for the other tree reduction rules.
%
%As the is not cyclic path in $\bb E$, the only possibility is that $\pi$ passes through an instance of the tree $\cc X\theta$, and this can only happen if the path enters either some $\mm E_{l}$ or $\cc F$ through some modular edge $(\gamma_{u}: Y^{d}, \gamma_{u+1}: Y^{\OV d})$ and then moves upwards through $\cc X\theta$ and ends up into a terminal node $\gamma_{u+2}: Z^{c}$ of some $\cc{\mathsf D}_{ji}[\cc X\mapsto \cc \bullet]$. Since $\pi$ is a cycle, there is then a path $\gamma_{u+2}\step\dots \step \gamma_{u}$. This path 
%
%
% some node $\gamma_{u}$ of some $\cc{D_{ji}}[\cc\bullet]$ 
\end{proof}

\begin{figure}
\adjustbox{scale=0.75, center}{$
\begin{tikzpicture}[baseline=-10]


\node[regular polygon,regular polygon sides=3, draw, shape border rotate=180] (a) at (0,0) { \ \ \ \ \ };
\node(aa) at (0.35,-1) {\small$\mm E_{l}$};
\node(y) at (0.6,0.7) {\small$\cc Y$};
\node(b) at (-0.6,0.7) {\small$\cc X$};

\node(xy) at (-1,-1.8) {\small$ X$};

\node(bz) at (-2, -1) {\small$\vec Z_{k}$};

\node(x) at (-1.3, -0.3) {\small$\mm X$};


\node[regular polygon,regular polygon sides=3, draw, shape border rotate=180] (v) at (-2.7,0.7) { \ \ \ \ \ };
\node(aa) at (-3.3,-0.3) {\small$\cc{\mathsf D}_{jk}[\cc X]$};

\node(z) at (-2.1, 1.4) {\small$\mm Z$};


\draw[thick] (xy) to (-0.05,-1.1);
\draw[thick] (xy) to (bz);
\draw[thick] (bz) to (x);
\draw[thick] (bz) to (-2.6,-0.4);

\draw[->, dotted, thick] (y) to [bend left=85] (b);
\draw[->, dotted, thick] (b) to [bend right=85] (x);
\draw[->, dotted, thick] (x) to [bend left=85] (z);

\end{tikzpicture}
\qquad \qquad\leadsto_{\cc X} \qquad \qquad 
\begin{tikzpicture}[baseline=30]


\node[regular polygon,regular polygon sides=3, draw, shape border rotate=180] (a) at (0,0) { \ \ \ \ \ };
\node(aa) at (0.35,-1) {\small$\mm E_{l}$};
\node(y) at (0.6,0.7) {\small$\cc Y$};
\node(b) at (-0.6,0.7) {\small$\bullet$};

\node(bb) at (-0.1, 1.4) {\small$\cc \bullet$};

\node(bz) at (-1, 1.4) {\small$Z_{k}$};

\node(br) at (-0.5, 2.1) {\small$\mm \bullet$};
\node[regular polygon,regular polygon sides=3, draw, shape border rotate=180] (v) at (-1.5,3.2) { \ \ \ \ \ };
\node(aa) at (-2.2,2.2) {\small$\cc{\mathsf D}_{jk}[\cc\bullet]$};

\node(z) at (-0.9, 3.9) {\small$\mm Z$};


\draw[thick] (b) to (bz);
\draw[thick] (b) to (bb);
\draw[thick] (br) to (bz);
\draw[thick] (-1.45,2.05) to (bz);

\draw[->, dotted, thick] (y) to [bend left=55] (b) to [bend left=10] (z);
\end{tikzpicture}$}
\caption{\small When $\bb E\leadsto_{\cc X}\bb E'$ an up-move in $\bb E'$ induces an alternate path in $\bb E$.}
\label{fig:cycle}
\end{figure}


\compositionality*
\begin{proof}%[Proof of Lemma \ref{rem:compositionality}]

If 
$\phi: \BV{B}\to \bb{Colors}$ and $\cc{\bb t}(B)$ is $\phi$-coherent, then  $\cc{\bb t}(A)$ is $\phi'$-coherent, where $\phi'$ is 
 the restriction $\phi|_{{\BV{A}}}$ of $\phi$ to $\BV{A}$. Moreover, it is clear that any cyclic alternate path in $\cc{\mathsf t}(A)$ yields a cyclic alternate path in $\cc{\mathsf t}(B)$.

The set $\BV{A[B/X]}$ can be identified with $V=\BV{A}\uplus \biguplus_{i=1}^{k}\BV{B}$, where $\uplus$ indicates disjoint union $k$ is the number of occurrences of $X$ in $A$.
Suppose $\cc{\bb t}(\forall X.A)$ is $\phi$-coherent and $\cc{\bb t}(B)$ is $\psi$-coherent, and let $\chi:=\phi|_{\BV{A}}\uplus \biguplus_{i=1}^{k}\psi$; we claim that $\cc{\bb t}(A[B/X])$ is $\chi$-coherent. First, any bound variable $\neq X$ in $A$ is coherent with any bound variable within any of the copies of $B$ in $A[B/X]$. Moreover, 
one can check that if an alternate path starts somewhere in the tree of $A[B/X]$ and enters the sub-tree 
corresponding to a copy of $B$, then the path must end within this sub-tree, since in 
any alternate path starting from (a copy of) $B$ all labels are bound variables of (this copy of) $B$, which are disjoint from all other bound variables.
%for all down- and up-moves $\alpha\step\beta$ with $\alpha$ in this sub-tree, $\beta$ belongs to the same sub-tree.
We deduce then that a cyclic alternate path in the tree of $A[B/X]$ can only be a cyclic alternate path in either $\cc{\mathsf t}(A)$  or in one copy of $\cc{\mathsf t}(B)$. Since both cases are excluded by assumption, no alternate cyclic path exists.
\end{proof}




==> applications.tex <==
% !TEX root = YonedaTryAgain.tex


In this section we discuss two interesting applications of the between finite characteristic polymorphism and $\mu,\nu$-types. 



\subparagraph*{Counting type inhabitants}

A natural application of Yoneda equalities is to \emph{count} the inhabitants of a type: given a (simpe type) $A$ with free variables $\vec X$, whenever $\forall \vec X.A$ rewrites into 
$ 0+ {1+\dots +1}=\sum_{i=1}^{k}1$, we deduce that $A$ has exactly $k$ proofs (up to equivalence). 


As a first example, we tested two simple and well-known criteria for \emph{unique inhabitation}, based on the properties of \emph{balancedness} and \emph{negative non-duplication} \cite{Aoto1999}. 
%A simple type is {balanced} if every variable occurs twice, once in positive and once in negative position, and is {negatively non-duplicated} if every variable occurs at most once in negative position. A type that is either balanced or  negatively non-duplicated has at most one inhabitant.
In the full paper we show that whenever a type $A$ satisfies either of these conditions, its universal closure $\forall \vec X.A$ rewrites into $1$ by Yoneda reduction. Moreover, we presented some simple types that do not satisfy neither of these conditions, but whose universal closure still rewrites into $1$.
%: for example the type 
%$(\cc Z\To \mm Y)\To \mm Z\To \mm Z\To \mm X\To \cc X$.


%
%
%based on proof-search (\cite{Zaoinc}).
%
%
% In fact, when a simple type $A$ has no occurrence of $X$, the isomorphism $A'=\forall X. (A\To \mm X)\To \cc X \equiv_{\varepsilon}A$ has a simple explanation in terms of proof-search: a closed $\eta$-long $\beta$-normal term of type $(A\To \mm X)\To \cc X$ must be of the form $\lambda f.fu$, where $u$  is a closed term of type $A$. Hence counting the terms of type $A'$ is tantamount as counting those of type $A$.
%
%This idea can be generalized to describe a connection between Yoneda type isomorphisms of the form 
%$\forall X. (\FFun{\cc X}{A}\To \mm X)\To \FFun{\cc X}{B}\equiv_{\varepsilon} \FFun{\cc X\mapsto \mu X.\FFun{\cc X}{A}}{B}$ and t
%
%
%The use of $\mu$-types in the proofs above to count the elements of a simple type might look puzzling at first. 
%Yet, we can justify this way of counting proofs by recalling that the proofs of a simple type can be counted by computing \emph{least fixpoints of polynomial equations} \cite{Zaoinc}. 


More generally, t


Let $\FFun{\cc X}{A}$ be the polynomial type $  \cc Y_{1} + (\cc X\times \cc Y_{2})$, and consider
the isomorphism $\forall X.A \equiv_{\varepsilon}\mu X. \cc Y_{1} + (\cc X\times \cc Y_{2})$, where 
$A=(\cc Y_{1}\To \mm X)\To (  \cc X\To \cc Y_{2}   \To \mm X)\To \cc X$.
A $\eta$-long $\beta$-normal term of type $A$ must be either of the form 
$\lambda f_{1}.\lambda f_{2}.f_{1}t$ or of the form $\lambda f_{1}.\lambda f_{2}.f_{2}uv$, where  $\Gamma\vdash t:\cc Y_{1}$, $\Gamma\vdash t:\cc X$ and $\Gamma\vdash u:\cc Y_{2}$, with $\Gamma=\{f_{1}:\mm Y_{1}\To \cc X, f_{2}: \mm X\To \mm Y_{2}\To \cc X\}$.
Hence, on the one hand we deduce that the number $|A|$ of inhabitants of $A$ must be a solution to the fixpoint equation
$|A|= |A_{Y_{1}}|+ (|A|\times |A_{Y_{2}}|)$, where $A_{Y_{i}}=(\cc Y_{1}\To \mm X)\To (  \cc X\To \cc Y_{2}   \To \mm X)\To \cc Y_{i}$, which yields $|A|=0$, since $|A_{Y_{i}}|=0$.
On the other hand, in terms of Yoneda type isomorphisms we can similarly deduce 
$\forall Y_{1}.\forall Y_{2}.\forall X.A \equiv_{\varepsilon}\forall Y_{1}.\forall Y_{2}.\mu X. \cc Y_{1} + (\cc X\times \cc Y_{2})\equiv_{\varepsilon} \mu X. 0 +(\cc X\times 0) \equiv 0$.
 

%
%
%\begin{remark}
%We will work here for simplicity in a fragment with simple types, sum, product, unit types and  $\mu$-types (hence without 0 nor $\nu$-types).
%\end{remark}
%%a Yoneda equality involving  $\int_{X}e$ (when $\kappa_{X}(e)\leq 3$) has a natural explanation in terms of proof-search.
% Write $e(\vec X)\in \C E_{0}$ as $X^{ \left ( \Pi_{i=1}^{p}X_{i}^{e_{i}}\right )\times \left ( \Pi_{j=1}^{q}X^{\left (\Pi_{ls=1}^{r_{j}}d_{jl}\right)}        \right) }$ and let $e'_{jl}:=d_{jl}^{ \left ( \Pi_{i=1}^{p}X_{i}^{e_{i}}\right )\times \left ( \Pi_{j=1}^{q}X^{\Pi_{j=1}^{r_{j}}d_{ij}}        \right) }$. Then a $\eta$-long $\beta$-normal term of type $e(\vec X)$ must be of the form
%$\lambda x_{1}\dots x_{p}\lambda y_{1}\dots y_{q}.y_{j}t_{1}\dots t_{q_{j}}$, where the terms $t'_{l}=\lambda x_{1}\dots x_{p}\lambda y_{1}\dots y_{q}.t_{l}$ have type $e'_{jl}$. Hence proving $e$ is tantamount as proving the $e_{jl}$. More precisely, 
%the number $|e|$ of proofs of $e$ can be computed from the numbers $|e'_{jl}|$ by the \emph{polynomial formula} $|e|= \sum_{j=1}^{q}\prod_{l=1}^{r_{j}}|e'_{jl}|$.
%
%Observe that $e$ might well coincide with some of the $e'_{jl}$: for instance, whenever $e(X)=X^{\left (X^{\pp(X)}\right)}$ for some polynomial $\pp(X)$, the reasoning above produces the \emph{recursive} polynomial formula $|e|= \pp(|e|)$. In fact, the number $|e|$ coincides with the \emph{least fixpoint} (computed in $\BB N\cup \{\infty\}$) of the polynomial formulas so obtained
%(e.g. for $\pp(X)=X+1$ we get $|e|=|e|+1$, which says that the type $\nat$ has infinitely many proofs). 
%The Yoneda equality $\int_{X}X^{\left (X^{\pp(X)}\right)}\simeq \mu X.\pp(X)$ allows then one to replace the least fixpoint $|e|=\pp(|e|)$ \emph{over $\BB N\cup \{\infty\}$} by a least fixpoint \emph{over types}.  
%

\subparagraph*{Simplifying type instantiations}


A second way to apply the correspondence between the types of $\NYY$ and \emph{initial algebras}/\emph{final coalgebras} is to compute transformation rules which allow to replace complex type instantiations by simpler ones.



For instance, suppose we define by induction a function $t: \nat \To (A \To B)$ by letting
 $t(0)$ be some fixed function $u: A\To B$ and 
$t({n+1})=F(t(n))$, where $F: (A\To B)\To (A\To B)$ maps a function $f$ onto $x\mapsto  h(f(x))$, for some fixed $h: B\To B$. 
Since the variable $x:A$ is used as a parameter, we could equivalently define $t$ by letting 
 $t_{x}(0)$ be some fixed $c=u(x):B$, and $t_{x}(n+1)$ be $h(t_{x}(n))$, so that $t(n)(x)=t_{x}(n)$.
Observe that in the first case we used an induction scheme employing the type $A\To B$, while in the second case we used an induction scheme employing the \emph{simpler} type $B$.  
More formally, the argument above shows the equivalence of the two polymorphic programs
$t_{1}=\lambda y.y (A\To B)( \lambda fx.h(fx))( u)$ and $t_{2}=\lambda y.\lambda x.y (B)( h)    (ux)$ of type $\nat\vdash A\To B$, the first involving a type instantiation on $A\To B$, the second a type instantiation on $B$. 

 This way of reasoning can be justified using the correspondence between $\mu$-types and \emph{initial algebras}.
In our example, using the fact that $\nat^{\flat}=\mu X.X+1$, we can reason in term of $X+1$-algebras: the two terms
correspond to $X+1$-algebra morphisms from $\nat$ to the $X+1$-algebras $(A\To B, \langle  \lambda x.h([\ ]x) ,u \rangle)$ and $(B, \langle h, ux\rangle)$. Now, since these two algebras are related by the $X+1$-algebra morphism $\rr{\TT E}= [\ ]x$, the equivalence
$t_{1}\simeq_{\varepsilon}t_{2}$ is an immediate consequence of the initiality of $\nat\equiv \mu X.X+1$. 

%
%
% We recall that a \emph{$T$-algebra} for a functor $T:\CTX_{\varepsilon}(\NYY)\to \CTX_{\varepsilon}(\NYY)$ is a pair $(A,\rr{\TT C})$ with $\rr{\TT C}: T(A)\vdash A$, and a \emph{$T$-algebra morphism} from $(A,\rr{\TT C})$ to $(B,\rr{\TT D})$ is a context $\rr{\TT E}:A\vdash B$ such that 
% $\rr{\TT E}[\rr{\TT C}] \simeq_{\varepsilon} \rr{\TT D}[T(\rr{\TT E})]$. 
% The \emph{initial $T$-algebra} $(\mu X.T, {\inn_{T}})$ is an initial object in the category of $T$-algebras and $T$-algebras morphisms. This means that for all $T$-algebra $(A,\rr{\TT C})$ there exists a \emph{unique} $T$-algebra morphism ${\ff}_{T}(\rr{\TT C}): \mu X.T\vdash  A$, corresponding to $T$-induction using the type $A$.
%  

The moral of this argument is that, whenever we have a $T$-algebra morphism which is an \emph{elimination context}, we can simplify the type of a $T$-induction. In the full paper we describe how this leads to devise a family of \emph{simplifying transformation rules} for $\NYY$ which replace a type instantiation by a simpler type.



Simplification rules can be used to show that the usual impredicative encoding $t\mapsto t^{\sharp}$ of $\NI$ into $\Nd$ (in fact, into $\NY$) can be turned into a fully \emph{predicative} one. 
The basic idea is to see a sum type $A+B$ as the initial algebra of the \emph{constant} functor
$F:\cc X\mapsto  A+B$. A $F$-algebra is then nothing but an arrow $\TT C:A+B \vdash C$, and an elimination context $\TT{El}:C\vdash D$ is trivially always a $F$-algebra morphism between $(C, \TT C)$ and $(D, \TT{El}\circ \TT C)$. 
By reasoning in this way we can deduce that simplification rules always apply the type instantiation occurring in $t^{\sharp}$, hence reducing it to a term containing only \emph{atomic} type instantiations.
%
%For example, for the type $\forall X.A=\forall X.(\FFun{\cc X}{P}\To \mm X)\To \cc X$ coding the initial algebra $\mu X.\FFun{\cc X}{P}$, $[\ ](C) t: \forall X.A\vdash C$, where $t: \FFun{\cc X\mapsto C}{P}\To C$,  encodes $\FFun{\cc X}{P}$-induction on $C$. 
%Now, whenever an elimination context
%$\rr{\TT{El}}:A\vdash B$ is a morphism of  two $\FFun{\cc X}{P}$-algebras  $(A,\TT C)$, $(B, \TT D)$, we can derive the simplifying rule 
%$$[\ ](A)\lambda x.\rr{\TT C}[x]  \simeq_{\varepsilon}   \Intro[  [\ ](B)\lambda x. \rr{\TT D}[x]   ] : \forall X.A\vdash C$$ 
%where $\TT{In}$ is any introduction context satisfying $ \rr{\TT I}\circ \rr{\TT E}\simeq_{\eta}[\ ]$, using the fact that initiality yields $\Elim[[\ ](A)\lambda x.\rr{\TT C}[x]] \simeq_{\varepsilon} [\ ](B)\lambda x.\rr{\TT D}[x]$. 
%
%
%
%
%When  $\FFun{\cc X}{P}$ is constant (i.e. it does not contain occurrences of $\cc X$) $\Elim$ is trivially \emph{always} a $\FFun{\cc X}{P}$-algebra morphism between $(A,\rr{\TT C})$ and $(B, \Elim[\rr{\TT C}])$. Hence the simplification $[\ ] (A)\lambda x.\rr{\TT C}[x] \simeq_{\varepsilon} \Intro[ [\ ] (B)\lambda x. \Elim[ \rr{\TT C}[x]]]$ holds in full generality. 


%


%
%
%) it was shown that the usual encoding $t\mapsto t^{\sharp}$ of $\NI$ into $\Nd$ (in fact, into $\NY$) can be turned into a \emph{predicative} encoding $t\mapsto t^{\sharp_{\bb{pred}}}$, in which the polymorphic terms $t^{\sharp_{\bb{pred}}}$ only contain \emph{atomic} type instantiations. 
%
%sing the simplification lemma we can deduce a stronger fact: the impredicative encoding $t^{\sharp}$ can be converted into a predicative one by applying program transformations ``atomizing'' all type instantiations.
%
%
%
%\begin{theorem}\label{genff}
%If $\Gamma\vdash_{\NI}  t:A$, then there exists a term ${t^{\downarrow}}$ containing only atomic type instantiations such that $\Gamma^{\sharp}\vdash_{\NY}t^{\downarrow}:A^{\sharp}$ and $ t^{\sharp} \simeq_{\varepsilon}{t^{\downarrow}}$. 
%\end{theorem}
%\begin{proof}
%For all $\Nd$-type $B$, with rightmost variable $Y$, we can always construct a pair of dual contexts $(\Elim, \Intro)_{B\vdash Y}$. 
%Observing that all universal types produced by the embedding of $\NI$ into $\NY$
%are pseudo-polynomials, using the reasoning above we can transform any type instantiation $t^{\sharp}$ into an atomic one.
%\end{proof}
%%
%






==> appstandard.tex <==
% !TEX root = YonedaTryAgain.tex



Let us call a $c$-eliminable variable $ X$ \emph{$c$-canceling} in the following cases:
\begin{itemize}
\item $\bb r_{X}$ is the root of a positive tree as in Fig. \ref{fig:11} left, where $c=\cc{\mathrm{blue}}$, $Y\neq X$ and no node in any sub-tree $\FFun{\cc X}{\mm F_{l}}$ has label $\cc X$;
\item $\bb r_{X}$ is the root of a positive tree as in Fig. \ref{fig:12} left, $c=\mm{\mathrm{red}}$ and no node in any sub-tree $\FFun{\mm X}{\mm F_{l}}$ has label $\mm X$;
\item $\bb r_{X}$ is the root of a negative tree as in Fig. \ref{fig:21} left, $c=\cc{\mathrm{blue}}$ and no node in any sub-tree $\FFun{\cc X}{\cc F_{l}}$ has label $\cc X$;
\item $\bb r_{X}$ is the root of a negative tree as in Fig. \ref{fig:22}, $c=\mm{\mathrm{red}}$, $Y\neq X$ and no node in any sub-tree $\FFun{\mm X}{\cc F_{l}}$ has label $\mm X$.
\end{itemize}

In fact, $X$ is $c$-canceling precisely when by applying a $X^{c}$-reduction step, the action of the substitution $\theta$ from Fig. \ref{fig:rewriting} is empty, so that the whole left-hand part of the tree, including some of its bound variables, is erased. 
Observe that, if $X$ is not $c$-canceling, and $\bb E\leadsto_{X^{c}}\bb E'$, then the application $ Y\mapsto g( Y)$ from a bound variable of $\bb E'$ to a bound variables of $\bb E$ from which $Y$ ``comes from'' is a \emph{surjective} function $g: \BV{\bb E'}\to \BV{\bb E}-\{X\}$.



A standard reduction $\bb E\stand^{*} \bb E'$ is said \emph{least-canceling} if for all $c$-canceling variable $X$, a reduction $\leadsto_{X^{c}}$ is performed only after all bound variables $ Y$ occurring above the node $\bb r_{X}$ are eliminated. 
Let us indicate by $\bb E\leadsto_{\bb{canc}}\bb E'$ that $\bb E$ reduces to $\bb E'$ by a sequence of least-canceling standard reductions.

\solvability*
\begin{proof}%[Proof of Theorem \ref{thm:solvability}]

Suppose $\bb E$ is coherent. From Lemma \ref{lemma:solvable} we deduce that if $\bb E\stand^{*} \bb E'$, then either $\bb E'\in \C P_{0}$ or $\bb E'\stand \bb E''$ for some $\bb E''$. Since sequences of standard reductions terminate, we deduce that $\bb E$ must in the end converge onto some simple tree.




Conversely, suppose $\bb E$ strongly converges under $\stand$. Since all standard reductions converge, there must be a converging least-canceling standard reduction $\bb E=\bb E_{0}\leadsto_{Y_{1}^{c_{1}}} \bb E_{1}\leadsto_{Y_{2}^{c_{2}}} \dots \leadsto_{Y_{n}^{c_{n}}}\bb E_{n}\in \C P_{0}$. 
Let $\delta(X)= \min\{i \mid G_{i}(Y_{i})= X\}$ and $\phi(X)=c_{\delta(X)}$. 
Using the fact that the variables $G_{i}(Y_{i})^{c_{i}}$ are pairwise coherent and include all bound variables of $\bb E$, one can check that $\delta$ and $\phi$ are well-defined and $\bb E$ is $\phi$-coherent.
%
%then any map of the form $X_{j}\mapsto d_{j}$, 
%where for some $1\leq i\leq n$, $G_{i}(Y_{i})=X_{j}$ and $d_{j}=c_{i}$, is a coherent valuation for $\bb E$.
\end{proof}



%
%
%
%Let us call a solvable variable $X$ \emph{canceling} if it does not occur in the terms $\bb E_{l}, \bb F$ (following the four possible configurations in Fig. \ref{fig:confs}). When we reduce a canceling variable, the action of the substitution $\theta$ is void, hence part of the tree, including some of its bound variables, are erased. 


%%[
%
%\begin{theorem}
%$\bb E$ is coherent iff there exists a coherent $\bb E'$ such that $\bb E \leadsto_{\bb{canc}}\bb E'$.
%\end{theorem}
%\begin{proof}
%
%
%\end{proof}
%
%
%\begin{remark}
%It is not true that a solvable tree $\bb E$ converges under any reduction. For instance [EXAMPLE].
%\end{remark}
%


==> balanced1.tex <==
% !TEX root = YonedaTryAgain.tex

%
%
%\begin{lemma}\label{lemma:occ}
%
%Suppose $\Gamma,x:A\vdash t:X$ holds. If  $\Gamma=\FFun{\mm X}{\Gamma}$ and  $A= \langle\FFun{\mm X}{A_{i}}\rangle_{i}\To\cc X$, then $t=\lambda y_{1}.\dots .\lambda y_{p}.xu_{1}\dots u_{k}$ and if $x$ occurs in one of the $u_{i}$, then there exist infinitely many distinct $\beta$-normal and $\eta$-long terms $v$ such that  $\Gamma,x:A\vdash v:X$ holds.
%In fact, if $u_{i}$ contains $x$, then since it is $\eta$-long it contains a subterm of the form $xw_{1}\dots w_{k}$, where $w_{i}$ cannot be $\beta\eta$-equivalent to $u_{i}$. Then by replacing $w_{i}$ with $u_{i}$ we obtain a distinct term $t_{1}$ such that $\Gamma, x:A\vdash t':X$ holds. It is clear that this process can be repeated yielding new terms $t_{2},t_{3},\dots$.
%%
%%
%% and $B=\FFun{\cc X}{B}$, then $\FFun{\cc X}{A_{i}}$ has no occurrence of $ \cc X$.%
%%
%%and a $\beta$-normal $\eta$-long term $t$ such that $\Gamma, x:A\vdash t: B$, either the $\FFun{\cc X}{A_{i}}$ have no occurrence of $ \cc X$, or $x$ does not occur in $t$.
%\end{lemma}
%\begin{proof}
%By defini
%
%
%We can suppose w.l.o.g. that in the claim above $t$ is $\beta$-normal and $\eta$-long. 
%%Suppose by way of absurdity that for some $t$, $\Gamma,x:A\vdash t:B$ holds.
%We argue by induction on the size of $t$. 
%$t$ must be of the form $x u_{1}\dots u_{n}$. 
%Suppose $\FFun{\cc X}{A_{i_{0}}}$ has an occurrence of $\cc X$. Then the $u_{i_{0}}$
%Since the $u_{i}$ are $\eta$-long, for 
%
%
%\end{proof}
%
%
%\begin{lemma}\label{lemma:occ}
%Given a context $\Gamma=\FFun{\mm X}{\Gamma}$, types $A= \langle\FFun{\mm X}{A_{i}}\rangle_{i}\To\cc X$ and $B= \FFun{\cc X}{B}$, and a $\beta$-normal $\eta$-long term $t$ such that $\Gamma, x:A\vdash t: B$, 
%
%
%either the $\FFun{\cc X}{A_{i}}$ have no occurrence of $ \cc X$, or $x$ does not occur in $t$.
%\end{lemma}
%\begin{proof}
%By induction  on the size of $t$. Let $t=\lambda \vec  y.yu_{1}\dots u_{k}$. Observe that the types $C_{i}$ of the variables $y_{i}$ are of the form $C_{i}= \FFun{\mm X}{C_{i}}$, while the types $D_{j}$ of the terms $u_{j}$ are of the form $\FFun{\cc X}{D_{j}}$. 
%%Observe that $D_{j}$ can contain an occurrence of $\cc X$ only if $x$ occurs in $u_{j}$. 
%%In fact, since $u_{j}$ is  $\eta$-long, $u_{j}$ has a subterm $\lambda \vec z.zv_{1}\dots v_{r}$ with a type of the form $E_{1}\To \dots \To E_{q}\To \cc X$. This is only possible if $z=x$, whence $x$ occurs in $u_{j}$. 
%
%Suppose now that some $A_{i}$ contains an occurrence of $\cc X$. Then $x$ cannot occur in any of the terms $\lambda\vec y.u_{j}$: this is clear if $\FFun{\cc X}{D_{j}}$ has no occurrence of $X$, while if $\cc X$ occurs in $\FFun{\cc X}{D_j}$, we can apply the induction hypothesis. 
%%
%%
%%, for $i=1,\dots,k$, because since $D_{j}=\FFun{\cc X}{D_{j}}$ we can apply the induction hypothesis to $\lambda\vec y.u_{j}$. 
%Moreover, if $y=x$, then some $D_{j}$ must contain an occurrence of $\cc X$, hence some $u_{j}$ contains $x$, which is impossible by what we just proved. We conclude that $x$ does not occur in $t$.
%\end{proof}
%

\unique*
\begin{proof}%[Proof of Proposition \ref{prop:unique}]
Write $A$ as $\langle A_{k}\rangle_{k\in K}\To X_{u}$ and 
suppose $t= \lambda x_{1}.\dots x_{\sharp K}. x_{v} t_{1}\dots t_{p}$ is a closed term of type $A$ in  $\eta$-long $\beta$-normal form. This forces
$A_{v}= \langle A_{jv}\rangle_{j\in J_{v}}\To X_{u}$, with $\sharp J_{v}=p$, and 
implies that the terms $t_{j}^{*}=\lambda x_{1}\dots x_{\sharp K}. t_{j}$ have type
$\langle A_{k}\rangle_{k\in K}\To A_{jv}$. 


We argue by induction on the size of $t$. 

\begin{itemize}
\item suppose $A$ is balanced. Since $X_{u}$ occurs positively in the rightmost position of $A$ and negatively in the rightmost position of $A_{v}$, it cannot occur in any other $A_{w}$, for $w\neq v$. We deduce that the variable $x_{v}$ cannot occur in any of the terms $t_{j}$.
Then, up to some $\beta\eta$-isomorphisms, we can write $\forall \vec X. A$ as 
$\forall \vec X_{v\neq u}.\forall X_{v}. \left( \langle A_{jv}\rangle_{j\in J_{v}}\To  \mm X_{u} \right) \To 
\left (\langle A_{w}\rangle_{w\neq v} \To \cc X_{u}\right)$, and by applying isomorphism $\equiv_{\cc X}$ we obtain the type 
$\forall \vec X_{v\neq u}. \langle A_{w}\rangle_{w\neq v} \To \prod_{j\in J_{v}}A_{jv} $. 


Since the terms $\lambda x_{1}\dots \hat{x}_{v}\dots x_{\sharp K}.t_{j}$ have the balanced type
$A_{j}^{*}=\langle A_{w}\rangle_{w\neq v}\To A_{jv}$, by the induction hypothesis we deduce $A_{j}^{*}\equiv_{\bb Y}1$, and thus   we deduce 
$\forall \vec X_{v\neq u}. \langle A_{w}\rangle_{w\neq v} \To \prod_{j\in J_{v}}A_{jv} 
\equiv_{\beta\eta}
\forall \vec X_{v\neq u}. \prod_{j\in J_{v}}A_{j}^{*}
\equiv_{\beta\eta}
\prod_{j\in J_{v}}\forall \vec X_{v\neq u}A_{j}^{*}
\equiv_{\bb Y} \prod_{j\in J_{v}}1
\equiv_{\beta\eta}1
$. 


\item Suppose $A$ is negatively non-duplicated; we will exploit the fact that $A$ admits at most one $\eta$-long $\beta$-normal term up to equivalence (see \cite{Aoto1999}).
We argue by induction that $A$ reduces to $1$ using $\beta\eta$-isomorphisms and isomorphisms of the form $\equiv_{X^{c}}$, where the variable $X$ occurs negatively exactly once.
 Since $X_{u}$ occurs negatively once in rightmost position of $A_{v}$, it can only occur positively in the $A_{jv}$ and negatively in the $A_{w}$ for $w\neq v$. 
 
 Moreover, we claim that $x_{v}$ cannot occur in the $t_{j}$. In fact, suppose some $t_{j}$ contains $x_{v}$. Since it is $\eta$-long  it contains a subterm of the form $x_{v}w_{1}\dots w_{p}$, where $w_{j}$ cannot be $\beta\eta$-equivalent to $t_{j}$. Then by replacing $w_{j}$ with $t_{j}$ in $t$ we obtain a new term $t_{1}$ of type $A$. It is clear that this process can be repeated yielding infinitely many distinct $\beta$-normal and $\eta$-long terms $t_{2},t_{3},\dots$ of type $A$. This is impossible because $A$ admits only one term up to $\beta\eta$-equivalence. 
%
% 
% Suppose $\Gamma,x:A\vdash t:X$ holds. If  $\Gamma=\FFun{\mm X}{\Gamma}$ and  $A= \langle\FFun{\mm X}{A_{i}}\rangle_{i}\To\cc X$, then $t=\lambda y_{1}.\dots .\lambda y_{p}.xu_{1}\dots u_{k}$ and if $x$ occurs in one of the $u_{i}$, then there exist infinitely many distinct $\beta$-normal and $\eta$-long terms $v$ such that  $\Gamma,x:A\vdash v:X$ holds.
% 
%In fact, if $u_{i}$ contains $x$, then since it is $\eta$-long%
% 
%  Moreover, $x_{v}$ cannot occur in the $t_{j}$, as a consequence of Lemma \ref{lemma:occ}.
 
 
 
Hence, up to some $\beta\eta$-isomorphisms, we can write $\forall \vec X. A$ as 
$\forall \vec X_{w\neq u}.\forall X_{v}. \left( \langle \FFun{\cc X_{u}}{A_{jv}}\rangle_{j\in J_{v}}\To \mm X_{u} \right) \To 
\left (\langle \FFun{\cc X_{u}}{A_{w}}\rangle_{w\neq v} \To \cc  X_{u}\right)$, and by applying $\equiv_{\cc X}$ we obtain the type 
$\forall \vec X_{w\neq u}. \langle \FFun{\cc X_{u}\mapsto \alpha}{A_{w}}\rangle_{w\neq v} \To\alpha$, where 
$\alpha=\mu X_{u}. \prod_{j\in J_{v}}\FFun{\cc X_{u}}{A_{jv}} $,
 which is $\beta\eta$-isomorphic to
$\forall \vec X_{w\neq u}. \langle \FFun{\cc X_{u}\mapsto \alpha}{A_{w}}\rangle_{w\neq v} \To \Pi_{j\in J_{v}}\FFun{\cc X\mapsto \alpha}{A_{jv}}$, and finally to  
  $\prod_{j\in J_{v}}\left(\forall \vec X_{w\neq u}. \langle \FFun{\cc X_{u}\mapsto \alpha}{A_{w}}\rangle_{w\neq v} \To \FFun{\cc X\mapsto \alpha}{A_{jv}}\right)$.


Since the terms $\lambda x_{1}\dots \hat{x}_{v}\dots x_{\sharp K}.t_{j}$ have the negatively non-duplicated type
$\FFun{\cc X_{u}}{A_{j}^{*}}=\langle \FFun{\cc X_{u}}{A_{w}}\rangle_{w\neq v}\To \FFun{\cc X_{u}}{A_{jv}}$, by the induction hypothesis we deduce $\forall \vec X.\FFun{\cc X_{u}}{A_{j}^{*}}\equiv_{\bb Y}1$
using $\beta\eta$-isomorphisms and isomorphisms of the form $\equiv_{X_{w}^{c}}$, where $w\neq v$, so we deduce that also $\forall \vec X_{w\neq u}\FFun{\cc X_{u}\mapsto \alpha}{A_{j}^{*}}\equiv_{\bb Y}1$ holds. We can then conclude
$\forall \vec X.A\equiv_{\bb Y} \prod_{j\in J_{v}}\forall \vec X_{v\neq u}\FFun{\cc X_{u}\mapsto \alpha}{A_{j}^{*}}
\equiv_{\bb Y} \prod_{j\in J_{v}}1
\equiv_{\beta\eta}1$.
\end{itemize}
\end{proof}

\begin{lemma}\label{lemma:depth}
Suppose  $A= \langle A_{i}\To X_{i}\rangle_{i\in L}\To U$ has free variables $X_{1},\dots, X_{n}$, where the $A_{i}$ are $\To$-free $\NImu$-types and $U$ is a closed type constructed using only 0 and 1. Then $\forall  X_{1}\dots \forall X_{n}.A\equiv_{\bb Y}U$. 

\end{lemma}
\begin{proof}
We argue by induction on the number of variables $X_{1},\dots, X_{n}$ freely occurring in $A$.
If $n$ is 0 then the list  $L$ is empty, so the claim is obvious. Otherwise, suppose $L$ has a first element $i_{0}$, so that 
$A$ can be written, up to some $\beta\eta$-isomorphism, as 
$ 
\langle \FFun{\cc X_{i_{0}}}{A_{u}}\To\mm X_{i_{0}}\rangle_{u}\To
\langle   \FFun{\cc X_{i_{0}} }{B_{v}}\To\mm Y_{v}\rangle_{v} \To  U$
where the $ \FFun{\cc X_{i_{0}} }{A_{u}}$ and  $ \FFun{\cc X_{i_{0}} }{A_{u}}$ are $\To$-free types  and $ Y_{v}\neq X$.
Then $\forall  X_{1}\dots \forall X_{n}.A\equiv_{\cc X_{i_{0}}}
\forall X_{1}\dots \widehat{\forall X}_{i_{0}}\dots \forall X_{n}.
\langle   \FFun{\cc X_{i_{0}} }{B_{v}}\theta\To\mm Y_{v}\rangle_{v} \To  U$, where
$\theta: \cc X_{i_{0}}\mapsto \mu X_{i_{0}}. \sum_{u}\FFun{\cc X_{i_{0}}}A_{u}$, so we can conclude by the induction hypothesis.
\end{proof}

\positive*
\begin{proof}%[Proof of Proposition \ref{prop:many}]
We will establish the following stronger claim. Let a \emph{quasi-polynomial} be a type of the form $\langle A_{k}\rangle_{k\in K}\To
\sum_{i=1}^{p}\prod_{j=1}^{p_{i}} u_{ij}$, where $p, p_{i}\geq 1$, the $A_{k}$ are simple types of depth $\leq 1$ (hence of the form $\langle X_{v_{k}}\rangle_{v_{k}}\To X_{k}$) and 
the $u_{ij}$ are either variables or 0,1. We claim that for any quasi-polynomial  $P[X_{1},\dots, X_{n}]$, if $P$ is positively non-duplicated, then  $\forall X_{1}\dots \forall X_{n}.P\equiv_{\bb Y}0+1+\dots +1$.

We argue by induction on the number of variables occurring among the $u_{ij}$.
%, with a sub-induction on the number of the $A_{k}$.

If all $u_{ij}$ are either $0$ or $1$, then any $A_{k}=\langle X_{v_{k}}\rangle_{v_{k}}\To X_{k}$ is $\beta\eta$-isomorphic to  $(\Pi_{v_{k}}X_{v_{k}})\To X_{k}$ so we can apply Lemma \ref{lemma:depth} yielding $\forall X_{1}\dots \forall X_{n}.P\equiv_{\bb Y}
\sum_{i=1}^{p}\prod_{j=1}^{p_{i}} u_{ij}\equiv_{\beta\eta}
0+1+\dots +1$.


Suppose now $u_{i_{0}j_{0}}=Z$. Since $P$ is positively non-duplicated, we can write $P$, up to some $\beta\eta$-isomorphisms, as 
$
\langle \langle \cc Z_{lm}\rangle_{l}\To \mm Z\rangle_{m}\To \langle B_{m'}\rangle_{m'}\To \sum_{i=1}^{p}\prod_{j=1}^{p_{i}} u_{ij}
$
where none of $Z_{lm}$ coincides with $Z$ and $Z$ does not occur in any of the $B_{m'}$. Then we deduce 
$\forall X_{1}\dots \forall X_{n}.P \equiv_{\cc Z}
\forall X_{1}\dots \widehat{\forall Z}\dots \forall X_{n}.
 \langle B_{m'}\rangle_{m'}\To \sum_{i=1}^{p}\prod_{j=1}^{p_{i}} u_{ij}\theta
$, where $\theta: \cc Z \mapsto \sum_{m}\prod_{l}\cc Z_{lm}$. Observe that the type  $\langle B_{m'}\rangle_{m'}\To \sum_{i=1}^{p}\prod_{j=1}^{p_{i}} u_{ij}\theta$
 is positively non-duplicated, has one variable less than $P$, and moreover, reduces using $\beta\eta$-isomorphisms to a type of the form $\langle B_{m'}\rangle_{m'}\To \sum_{i=1}^{p'}\prod_{j=1}^{p'_{i}} v_{ij}$, where the $v_{ij}$ are among $0,1,X_{1},\dots, \widehat Z, \dots, X_{n}$. We can thus apply the induction hypothesis.
\end{proof}


%We argue by induction on the number of the $A_{k}$.
%If $P= \sum_{i=1}^{p}\prod_{j=1}^{p_{i}}\cc Y_{ij}$, then  by applying the isomorphism $\equiv_{\cc Y_{i}}$, we deduce $\forall X_{1}\dots \forall X_{n}.P\equiv_{\bb Y}  \sum_{i=1}^{p}\prod_{j=1}^{p_{i}}u_{ij}\equiv_{\beta\eta}0+1+\dots +1$, where the $u_{ij}$ are either $0$ or $1$.
%
%Suppose now there is at least one type of the form $A_{k_{0}}$ in $P$ and let $X_{u}$ be its rightmost variable. Since $A_{k_{0}}$ has depth at most 1, it is of the form  $\langle \mm Z_{lk_{0}}\rangle_{l}\To \cc X_{u}$, for variables $Z_{lk_{0}}$ and $X_{k_{0}}$. Then, by splitting the $A_{k}$ into those whose rightmost variable is $X_{u}$ and those whose rightmost variable is not $X_{u}$, we can write 
% $P$, up to some $\beta\eta$-isomorphism as 
%$
%\langle \langle \cc Z_{lm}\rangle_{l}\To \mm X_{u}\rangle_{m}\To \langle B_{s}\rangle_{s}\To \sum_{i=1}^{k}\prod_{j=1}^{k_{i}}\cc Y_{ij}
%$. 
%Since $W_{k_{0}}$ occurs positively only once, three cases arise:
%\begin{itemize}
%\item There is no occurrence of $\cc X_{u}$ or the unique occurrence of $\cc X_{u}$ is among the $Z_{lk}$: 
% then $\forall X_{1}\dots \forall X_{n}.P \equiv_{\cc X_{u}}
%\forall X_{1}\dots \widehat{\forall X}_{u}\dots \forall X_{n}.  \langle B_{s}\rangle_{s}\To \sum_{i=1}^{k}\prod_{j=1}^{k_{i}}\cc Y_{ij}
%$, so we can apply the induction hypothesis. 
%
%
% 
%\item The unique occurrence of $\cc X_{u}$ occurs in one of the $B_{s}$, say $B_{s_{0}}$; then $B_{s_{0}}$ can be written, up to some $\beta\eta$-isomorphisms, as $\mm X_{u}\To B'_{s}$, and then by applying $\equiv_{\cc X_{u}}$ we reduce
%$ \forall X_{1}\dots \forall X_{n}.P $ as follows:
%\begin{align*}
%& \equiv_{\cc X_{u}} 
%\forall X_{1}\dots \widehat{\forall X}_{u}\dots \forall X_{n}.  
%\Big (  \big( \sum_{m}\prod_{l}\cc Z_{lm}\big) \To B'_{s}\Big)  
%\To
%\langle B_{s}\rangle_{s\neq s_{0}}\To \sum_{i=1}^{k}\prod_{j=1}^{k_{i}}\cc Y_{ij} \\
%& \equiv_{\beta\eta}
%\forall X_{1}\dots \widehat{\forall X}_{u}\dots \forall X_{n}.  
%\Big  (\prod_{m}   \big ( \langle \cc Z_{lm}\rangle_{l}\To B'_{s}    \big)    \Big)
%\To
%\langle B_{s}\rangle_{s\neq s_{0}}\To \sum_{i=1}^{k}\prod_{j=1}^{k_{i}}\cc Y_{ij} 
%\end{align*}
%
%\item The unique occurrence of $\cc X_{u}$ is among the $Y_{ij}$;
%\end{itemize}
%
%
%Then, by applying an isomorphism $\equiv_{\cc W_{k_{0}}}$, we reduce $P$ to 
%$
%\langle \langle Z_{lk}\rangle_{l}\To W_{k_{0}}\rangle_{m}\To \langle B_{m'}\rangle_{m'}\To \sum_{i=1}^{k}\prod_{j=1}^{k_{i}}Y_{ij}
%$
%
%Again, if all $X_{ij}\in \{0,1\}$, then one can check that $\forall X_{1}\dots \forall X_{n}.P\equiv_{\beta\eta}0+1+\dots+1$, so we are done. Otherwise, pick a variable $X_{i_{0}j_{0}}$. If $X_{i_{0}j_{0}}$ does not occur negatively in $P$, then you can apply an isomorphism $\equiv_{\cc X_{i_{0}j_{0}}}$, transforming $\forall X_{1}\dots \forall X_{n}.P $ onto
%$\forall X_{1}\dots \widehat{X}_{i_{0}j_{0}}\dots \forall X_{n}.\langle A_{k}\rangle_{k}\To
%\sum_{i=1}^{p}\prod_{j=1}^{p_{i}}(X_{ij}\theta)$, where $\theta:X_{i_{0}j_{0}}\mapsto 0$, and we can conclude by the induction hypothesis.
%Suppose now $X_{i_{0}j_{0}}$ occurs negatively in some $A_{k}$. Since $d(A_{k})\leq 1$, it must be 
%$A_{k}=  \langle \mm Y_{m}\rangle_{m}\To \cc X_{i_{0}j_{0}}$, with the $Y_{m}\neq X_{i_{0}j_{0}}$. Then $P$ can be written, up to some $\beta\eta$-isomorphism as 
%$
%\langle \langle Y_{rm}\rangle_{r}\To X_{i_{0}j_{0}}\rangle_{m}\To \langle B_{s}\rangle_{s}\To \sum_{i=1}^{k}\prod_{j=1}^{k_{i}}X_{ij}
%$
%where $m\geq 1$.
%Since $P$ is positively non-duplicated, it follows that none of the $Y_{rm}$ can be $X_{i_{0}j_{0}}$, nor any $B_{s}$ can contain $X_{i_{0}j_{0}}$, so we can apply the rule $\equiv_{\cc X_{i_{0}j_{0}}}$, yielding the type
%$
%\langle B_{s}\rangle_{s}\To \sum_{i=1}^{p}\prod_{j=1}^{p_{i}}(X_{ij}\theta)
%$
%where $\theta: X_{i_{0}j_{0}}\To \sum_{r}\prod_{m}Y_{rm}$. Using $\beta\eta$-isomorphisms we can then 
%turn $\sum_{i=1}^{p}\prod_{j=1}^{p_{i}}(X_{ij}\theta)$ into a type of the form $\sum_{i'=1}^{p'}\prod_{j'=1}^{p'_{i}}X_{i'j'}$, so that we obtain that a $\forall X_{1}\dots \forall X_{n}.P$ is isomorphic to
%$\forall X_{1}\dots \widehat{X}_{i_{0}j_{0}}\dots \forall X_{n}.\langle A_{k}\rangle_{k}\To
%\sum_{i'=1}^{p'}\prod_{j'=1}^{p'_{i}}X_{i'j'}$, and we can again apply the induction hypothesis.
%%
%
%
% 
%% 
%
%
%Let $P=\langle A_{k}\rangle_{k}\To
%\sum_{i=1}^{k}\prod_{j=1}^{k_{i}}X_{ij}$ and  $t$ be a term of type $P$ normal with respect to $\beta$ and commutative conversions. Then, up to some $\eta$-expansion step, $t$ must be of the form
%$\lambda x_{1}\dots x_{\sharp K}. \iota^{\sharp I}_{i_{0}}(\mathsf{prod}^{\sharp J_{i}}( t_{1},\dots, t_{k_{i}} )  )$, where  $t_{j}= x_{l_{j}}u^{j}_{1}\dots u^{j}_{p_{j}}$.
%
%Fix a value $j_{0}$. Since $t_{j_{0}}$ has type $X_{i_{0}j_{0}}$ it follows that $A_{i_{0}}= \langle Y_{m}\rangle_{m}\To X_{i_{0}j_{0}}$, where $u^{j_{0}}_{m}$ has type $Y_{m}$. Then $P$ can be rewritten, up to some $\beta\eta$-isomorphism as 
%$
%\langle \langle Y_{rm}\rangle_{r}\To X_{i_{0}j_{0}}\rangle_{m}\To \langle B_{s}\rangle_{s}\To \sum_{i=1}^{k}\prod_{j=1}^{k_{i}}X_{ij}
%$
%where $m\geq 1$.
%Since $P$ is positively non-duplicated, it follows that none of the $Y_{rm}$ can be $X_{i_{0}j_{0}}$, nor any $B_{s}$ can contain $X_{i_{0}j_{0}}$, 
% so we can apply the rule $\equiv_{\cc X_{i_{0}j_{0}}}$, yielding the type
%$
%\langle B_{s}\rangle_{s}\To \sum_{i=1}^{k}\prod_{j=1}^{k_{i}}(X_{ij}\theta)
%$
%where $\theta: X_{i_{0}j_{0}}\To \sum_{r}\prod_{m}Y_{rm}$.
%
%


==> betaetainvariance.tex <==
% !TEX root = YonedaTryAgain.tex

We show that the tree-representation of $\Nd$-types from Section 4 is invariant under $\beta\eta$-isomorphisms.
The $\beta\eta$-isomorphisms of $\Nd$ are completely axiomatized as shown in Fig. \ref{fig:isond}. A type $A$ of $\Nd$ is \emph{in normal form} (shortly, \emph{in NF}) if $A= \forall \vec Y.A_{1}\To  \dots \To  A_{n} \To X$ where each variable in $\vec Y$ occurs at least once in $A_{1}\To  \dots \To  A_{n} \To X$, and the types $A_{1},\dots, A_{n}$ are in normal form. Let $\bb{NF}(\Nd)$ be the set of $\Nd$-types in NF.

Given $A, B\in \bb{NF}(\Nd)$, with $A= \forall \vec Y.A_{1}\To  \dots \To  A_{n} \To X$ and 
$B= \forall \vec Z.B_{1}\To  \dots \To  B_{m} \To X'$, let $A \sim B$ when $n=m$, $\vec Y=\vec Z$, $X=X'$ and there exists 
$\sigma\in \F S_{n}$ such that $A_{i}\sim B_{\sigma(i)}$ for $i=1,\dots,n$. 

\begin{lemma}\label{lemma:nf}
\begin{itemize}
\item[i.] For all $A\in \Nd$, there exists a type $\bb{NF}(A)\in \bb{NF}(\Nd)$ such that $A\equiv_{\beta\eta}\bb{NF}(A)$.
\item[ii.] For all $A,B\in \Nd$, $A\equiv_{\beta\eta} B$ iff $\bb{NF}(A) \sim \bb{NF}(B)$.

\end{itemize}
\end{lemma}
\begin{proof}
Claim $i.$ is a consequence of applying the isomorphisms $\forall X.A\equiv_{\beta\eta} A$ when $X$ does not occur in $A$ and the isomorphisms 
 $A\To \forall X.B \equiv_{\beta\eta} \forall X. A\To B$ to push quantifiers in leftmost position. Claim $ii.$ follows then since the only other isomorphism rule is the permutation $A\To (B \To C) \equiv_{\beta\eta} B\To (A \To C)$.
\end{proof}

The definition of the tree-type $\cc{\mathsf t}(A)$ only depends on $\bb{NF}(A)$. Moreover, it can be checked by induction on $A$ that $\bb{NF}(A)\sim \bb{NF}(B)$ holds iff $\cc{\mathsf t}(A)=\cc{\mathsf t}(B)$. Hence, we deduce from Lemma \ref{lemma:nf} that $A\equiv_{\beta\eta} B$ iff $\cc{\mathsf t}(A)= \cc{\mathsf t}(B)$.

%
%
%We now extend the definition of $\cc{\bb t}(A)$ to the types of $\NImu$. We call a $\NImu$-type a \emph{base type} if its main type constructor is neither $\forall$ nor $\To$.
%A $\NImu$-type  is \emph{in normal form} (shortly, \emph{in NF}) if $A= \forall \vec X.A_{1}\To  \dots \To  A_{n} \To C$ where 
%each of the variables $\vec X$ occur at least once in $A_{1}\To  \dots \To  A_{n} \To C$, the types $A_{1},\dots, A_{n},C$ are in normal form and $C$ is a base type. 
%
%We can argue similarly to Lemma \ref{lemma:nf} to show that any $\Ntot$-type $A$ is $\beta\eta$-isomorphic to a type $\bb{NF}(A)$ in normal form. We can now define $\cc {\bb t}(A)$ as follows:
%
%\begin{itemize}
%\item if $A$ is a base type, then 
% 
% 
% $\cc {\bb t}(0)= \B{\cc 0} \qquad \cc {\bb t}(1)= \B{\cc 1}\qquad\cc {\bb t}(B+C)=$ \adjustbox{scale=0.8}{$\begin{tikzpicture}[baseline=-10pt]
%%\node (a0) at (-0.7,0.1 ) {\small$\cc\bullet$};
%
%\node (a) at (0,0.1 ) {\small$\cc {\bb t}(B)$};
%\node (aa) at (0.7,0.1) {\small$\mm\bullet$};
%\node(aaa) at (0.35,-0.5) {\small$\emptyset$}; 
%
%\node (b) at (1.5,0.1 ) {\small$\cc {\bb t}(C)$};
%\node (bb) at (2.2,0.1) {\small$\mm\bullet$};
%\node(bbb) at (1.85,-0.5) {\small$\emptyset$}; 
%
%\node(d) at (3, -0.5) {\small$\cc \bullet$};
%
%\node(c) at (1.85, -0.9) {\small$\bullet$};
%
%%\draw (a0) to (aaa);
%
%\draw (a) to (aaa);
%\draw (aa) to (aaa);
%\draw (b) to (bbb);
%\draw (bb) to (bbb);
%\draw (a) to (aaa);
%\draw (c) to (aaa);
%\draw (c) to (bbb);
%\draw (c) to (d);
%\end{tikzpicture}
%%\AXC{\small$\cc{\bb E}_{11}$}
%%\AXC{\small$\cc{\bb E}_{12}$}
%%\BIC{\small$\mm \bullet$}
%%\AXC{\small$\cc{\bb E}_{23}$}
%%\UIC{\small$\mm \bullet$}
%%\RL{\tiny$\forall \bullet$}
%%\BIC{\small$\cc \bullet$}
%%\DP
%$}
%
%$
%\cc {\bb t}(B\times C)=$ \adjustbox{scale=0.8}{$\begin{tikzpicture}[baseline=-10pt]
%%\node (a0) at (-0.7,0.1 ) {\small$\cc\bullet$};
%
%%\node (a) at (0,0.1 ) {\small$\cc {\bb t}(B)$};
%%\node (aa) at (0.7,0.1) {\small$\mm\bullet$};
%%\node(aaa) at (0.35,-0.5) {\small$\emptyset$}; 
%
%\node (a) at (0.7,0.1 ) {\small$\cc {\bb t}(B)$};
%\node (b) at (1.5,0.1 ) {\small$\cc {\bb t}(C)$};
%\node (bb) at (2.2,0.1) {\small$\mm\bullet$};
%\node(bbb) at (1.85,-0.5) {\small$\emptyset$}; 
%
%\node(d) at (3, -0.5) {\small$\cc \bullet$};
%
%\node(c) at (2.42, -0.9) {\small$\bullet$};
%
%%\draw (a0) to (aaa);
%
%\draw (a) to (bbb);
%%\draw (aa) to (aaa);
%\draw (b) to (bbb);
%\draw (bb) to (bbb);
%%\draw (a) to (aaa);
%%\draw (c) to (aaa);
%\draw (c) to (bbb);
%\draw (c) to (d);
%\end{tikzpicture}
%%\AXC{\small$\cc{\bb E}_{11}$}
%%\AXC{\small$\cc{\bb E}_{12}$}
%%\BIC{\small$\mm \bullet$}
%%\AXC{\small$\cc{\bb E}_{23}$}
%%\UIC{\small$\mm \bullet$}
%%\RL{\tiny$\forall \bullet$}
%%\BIC{\small$\cc \bullet$}
%%\DP
%$}	
%
%
%\end{itemize}




==> eliminable.tex <==
% !TEX root = YonedaTryAgain.tex

\normalform*
\begin{proof}%[Proof of Proposition \ref{prop:normalform}].
If $ X$ is $\cc{\mathrm{eliminable}}$ in a positive tree $\cc{\mathsf E}=$ 
\adjustbox{scale=0.7}{\begin{tikzpicture}[baseline=-20]
	\node(a) at (0,0) {\small $\Big \{ \mm{\bb E}_{i}\Big \}_{i\in I}$};
	\node (b) at (1.4,0) {\small$ \cc X$};
	\node (c) at (0.7,-0.8) {\small${ \vec{ Y}} X$};
	\draw (a) to (c);
	\draw (b) to (c);
	\end{tikzpicture} }, 
	then let us split the negative subtrees $\mm{\bb E}_{i}$ into those which do not contain terminal nodes  with label $\mm X$, that we indicate as $\FFun{\cc X}{\mm{\mathsf F}_{l}}$, and those which contain a (necessarily unique) modular node of label $\mm X$, that we indicate
as $\mm{\bb G}_{k}$. Since $\mm{\bb G}_{k}$ contains a unique modular node $\alpha_{k}:\mm X$ which is no more than two edges far away from the root of $\cc{\mathsf E}$, then $\mm {\bb G}_{k}$ is of the form 	\adjustbox{scale=0.8}{\begin{tikzpicture}[baseline=-20]
	\node(a) at (0,0) {\small $\Big \{ \FFun{\cc X}{\cc{\mathsf D}_{jk}}\Big \}_{i\in I}$};
	\node (b) at (1.4,0) {\small$ \mm X$};
	\node (c) at (0.7,-0.8) {\small${\vec{  Z}_{k}}$};
	\draw (a) to (c);
	\draw (b) to (c);
	\end{tikzpicture} }, where possibly $I= Z_{k}=\emptyset$, (so that $\mm{\bb G}_{k}=\mm X$). 


If $X$ is $\mm{\mathrm{eliminable}}$ in a positive tree $\cc{\mathsf E}=$ 
\adjustbox{scale=0.7}{\begin{tikzpicture}[baseline=-20]
	\node(a) at (0,0) {\small $\Big \{ \mm{\bb E}_{i}\Big \}_{i\in I}$};
	\node (b) at (1.4,0) {\small$ \cc X$};
	\node (c) at (0.7,-0.8) {\small$\vec{ Y}X$};
	\draw (a) to (c);
	\draw (b) to (c);
	\end{tikzpicture} }, 
	then, since all nodes $\alpha:\cc X$ are modular, it must be $\cc Y\neq \cc X$. Let us split the positive subtrees $\cc{\mathsf E}_{i}$ into those which do not contain terminal nodes  with label $\cc X$, that we indicate as $\FFun{\mm X}{\mm{\mathsf F}_{l}}$, and those which contain a (necessarily unique) modular node of label $\cc X$, that we indicate
as $\cc G_{k}$. Since $\cc G_{k}$ contains a unique modular node $\alpha_{k}:\cc \alpha$ which is no more than two edges far away from the root of $\cc{\mathsf E}$, then $\cc G_{k}$ is of the form 	\adjustbox{scale=0.8}{\begin{tikzpicture}[baseline=-20]
	\node(a0) at (-1.5,0) {\small$\mm X$};
	\node(a) at (0,0) {\small $\Big \{ \FFun{\mm X}{\cc{\mathsf D}_{jk}}\Big \}_{i\in I}$};
	\node (b) at (1.4,0) {\small$ \FFun{\mm X}{\cc{\mathsf E}_{k}}$};
	\node (c) at (0.7,-0.8) {\small${\vec{{ Z}}_{k}}$};
	\draw (a) to (c);
	\draw (b) to (c);
		\draw (a0) to (c);
	\end{tikzpicture} }.
	
	The two cases with a negative tree are described in a dual way (i.e. by switching blue and red everywhere).
\end{proof}



\termination*
\begin{proof}%[Proof of Proposition \ref{prop:termination}]
Let $K$ be the number of terminal nodes of $\bb E$ and, for all bound variable $X_{i}$ of $\bb E$, let $K_{i}$ be the number of terminal nodes of the subtree $\bb E_{i}$ of $\bb E$ with root $\bb r_{X_{i}}$.
Fix some $s> K^{2}$ and let $\mu(\bb E)$ be the sum of all $s^{K_{i}}$, for all bound variable $X_{i}$.
%, so that $\mu(\bb E)\leq  N (cK)^{2K}$. 
If $\bb E \leadsto_{X_{i}^{c}} \bb E'$, then the elimination of $X_{i}$ comes at the cost of possibly duplicating the bound variables which are at distance at least one from the root of $\bb E_{i}$. These are no more than $K_{i}$ and can be duplicated for no more than $K_{i}$ times. Since for each such variable $j$, it must be $K_{j}< K_{i}$, we deduce that $\mu(\bb E')$ is obtained by replacing  in $\mu(\bb E)$ the summand $s^{K_{i}}$ by a sum of no more than $K_{i}^{2}$ summands which are bounded by $s^{K_{i}-1}$. Hence, if we write $\mu(\bb E)$ as $ a+ s^{K_{i}}$, then $\mu(\bb E')  \leq a+ K_{i}^{2}s^{K_{i}-1} < a + s^{K_{i}}=\mu(\bb E)$. We deduce that the measure $\mu(\bb E)$ strictly decreases under reduction, and so, if an infinite sequence of reductions exists, then after a large enough number of step one must obtain a tree $\bb E'$ such that  $\mu(\bb E')<0$, which is impossible.
\end{proof}


We indicate a standard reduction as $\bb E\stand^{*} \bb E'$.


\begin{lemma}\label{lemma:solvable}
If $\bb E$ is coherent, and $\bb E\stand^{*} \bb E'$, then $\bb E'$ is coherent.
\end{lemma}
\begin{proof}
%[Proof of Lemma \ref{lemma:solvable}]


For any node $\alpha$ of $\bb E'$ there exists a unique node, that we indicate as $g(\alpha)$, from which 
 $\alpha$ ``comes from'' through the reduction step. Moreover, for each bound variable $Y\in \BV{\bb E'}$ there exists a unique bound variable $g(Y)\in \BV{\bb E}$ from which $Y$ ``comes from'' through the reduction step.


We indicate as $\alpha\preceq \beta$ the tree-order relation on the nodes of $\bb E$ (so that the root of $\bb E$ is the minimum node). 
Suppose $\bb E$ is $\phi$-coherent and $\bb E\leadsto_{X^{\phi(X)}} \bb E'$. 
We will show that $\bb E'$ is
 $\phi\circ g$-coherent.
 
Let $\mathsf{F}$ be the sub-tree of $\bb E$ with root $\bb r_{X}$, fix a variable $Y$ in $\BV{\bb E'} $.
 We must consider four possible cases, corresponding to the four reduction rules. Each rule requires itself four subcases. We only consider the case of the first rule (hence with $\bb E$ positive), as the other three cases can be proved in a similar way.
\begin{description}
\item[($\cc{\mathsf{F}}\leadsto_{\cc X}\cc{\mathsf F'}$)]   We first show that $Y$ is $\phi(g(Y))$-eliminable in $\cc{\mathsf{F}}'$, by showing that any modular node $\alpha: g(Y)$ in $\cc{\mathsf{F}}$ is transformed into a modular node $\beta:Y$ in $\cc{\mathsf{F}}'$. We argue by considering the relative position of $\bb r_{X}$ and $\bb r_{Z}$ in $\cc{\mathsf E}$:
	\begin{description}
	\item[($\bb r_{X}=\bb r_{g(Y)}$)] Since $\cc X$ and $g(Y)^{\phi(g(Y))}$ are coherent in $\cc{\mathsf E}$, and all nodes $\alpha:g(Y)^{\OV{\phi(g(Y))}}$ are modular, each such node $\alpha$ must be a terminal node of some of the $\FFun{\cc X}{\mm{\mathsf F}_{l}}$
	(see Fig. \ref{fig:11}). In fact, if $\alpha$ were a terminal node of some $\FFun{\cc X}{\cc{\mathsf D}_{jk}}$, then either $\FFun{\cc X}{\cc{\mathsf D}_{jk}}=g(Y)^{\OV{\phi(g(Y))}}$, which contradicts the assumption that $\cc X$ and $g(Y)^{\phi(g(Y))}$ are coherent, or its distance from $\bb r_{X}=\bb r_{g(Y)}$ is greater than 2, against the assumption that $\alpha$ is modular. 
	Now, since all nodes in $\FFun{\cc X}{\mm{\mathsf F}_{l}}$ which are not labeled with $\cc X$ are not ``moved'' by the reduction rule (see Fig. \ref{fig:11}), and no new node labeled $g(Y)^{\phi(g(Y))}$ is created by $\theta$ (since otherwise it should come from a node with same label in some $\FFun{\cc X}{\cc{\mathsf D}_{jk}}$), all nodes $\alpha:Y^{\OV{\phi(g(Y))}}$ in $\cc{\mathsf F'}$ are modular, whence $Y$ is $\phi(g(Y))$-eliminable in $\mathsf{F}'$. 
	



%
%
% This is clear if the the transformation $\cc V \leadsto_{\cc X}\cc{V'}$ creates no new parallel terminal node.
%Otherwise, the only way in which the transformation $\cc V \leadsto_{\cc X}\cc{V'}$ can introduce new parallel terminal nodes (hence new potential conflicts) is if $\theta$ replaces the terminal nodes labeled $\cc X$ by a terminal node, and this is possible only if
%$k=1$, for some $j\leq p_{1}$, $\cc{T_{1j}}=Y^{c}$, and some $\mm{U_{i}}$ contains two parallel nodes $\alpha: \cc X, \beta: Z^{d}$. 


%
%Then in this case $Y^{\OV c}$ is in conflict with $\cc X$ in $\mathsf V$, so it must be $\phi(Y)=c$, and 
%$\C C(\mathsf T')= \C C(\mathsf T)- \C C_{X}(\mathsf T) \cup \{ (Y^{\OV c}, Z^{\OV d})\}$. Hence if we let $\psi: \BV{\mathsf T'}\to C$ be the restriction of $\phi$ to $\BV{\mathsf T'}$, we are sure to produce no conflict in $\mathsf T'$.
%

	
	\item[($\bb r_{X}\prec\bb r_{g(Y)}$)] First, if $\bb r_{g(Y)}$ occurs within either the $\FFun{\cc X}{\cc{\mathsf D}_{jk}}$ or the $\FFun{\cc X}{\mm{\mathsf F}_{l}}$, then one can check that, by the transformation from $\cc{\mathsf{F}}$ to $\cc{\mathsf F'}$, the relative positions between the nodes $g(\alpha): g(Y)^{c}$ and $\bb r_{g(Y)}$ in $\bb E$ coincide with the relative positions between the nodes $\alpha$ and $\bb r_{Y}$, and thus all modular nodes $\delta:g(Y)^{\OV{\phi(g(Y))}}$ in $\cc{\mathsf{F}}$ yield modular nodes $\delta':Y^{\OV{\phi(g(Y))}}$ in $\cc{\mathsf{F}}'$.
	
		
	Suppose now $g(Y)$ is among some set $\vec Z_{k}$ (see Fig. \ref{fig:11}). One can check that for all node $\delta:g(Y)^{\OV{\phi(g(Y))}}$ occurring in $\mathsf{F}$ within one of the $\FFun{\cc X}{\cc{D}_{jk}}$, if, in the transformation of $\cc{\mathsf{F}}$ in $\cc{\mathsf{F}}'$, $\delta$ is transformed into $\delta'$, then $d(\delta, \bb r_{g(Y)})$ in $\cc{\mathsf E}$ is the same as $d(\delta', \bb r_{Y})$ in $\cc{\mathsf E}'$. Moreover, it is clear that $\delta'$ cannot be the head of the sub-tree rooted in $\bb r_{Y}$, and that if $\delta$ has no parallel node with same label, so does $\delta'$. Hence, if $\delta$ is modular, so is $\delta'$.
	
%	. Then the transformation $\cc V\leadsto \cc{V'}$ does not alter the distance between $\delta$ and $\gamma_{Y}$, which remains less than $2$, it cannot create new parallel terminal nodes to $\delta$, nor it can move $\delta$ in the position of head of $\gamma_{X}$, so we must conclude that any such $\delta$ is moved into traverse node in $\mathsf T'$. Since the transformation cannot create other nodes of label $Y^{\OV{\phi(Y)}}$, we deduce that $\kappa_{Y}(\mathsf T')$ is still finite. 

	
	
	\item[($\bb r_{g(Y)}\prec\bb r_{X}$)] 
	If a modular node $\delta: g(Y)^{\OV{\phi(g(Y))}}$ in $\cc{\mathsf E}$ is transformed into some node $\delta': Y^{\OV{\phi(Y)}}$ in $\cc{\mathsf E}'$, then $\delta'$ is modular too. In fact, no such $\delta$ can be actually moved by the reduction rule, since the only possibilities are that 
		either $\delta\prec \bb r_{X}$ or $\delta$ coincides with one of the $\FFun{\cc X}{\mm{\mathsf F}_{l}}$.
		Since neither the node $\bb r_{Y}$ is moved, we deduce that $\delta'$ has the same distance from $\bb r_{g(Y)}$ than $\delta$ has from $\bb r_{g(Y)}$, that it has no parallel node with same label and cannot be the head of the sub-tree rooted in $\bb r_{Y}$, whence $\delta'$ is modular.
		
			
	 
	
	\item[($\bb r_{g(Y)}\not\preceq\bb r_{X},\bb r_{X}\not\preceq\bb r_{g(Y)}$]
	We can argue as in the case above, since the transformation from $\cc{\mathsf{F}}$ to $\cc{\mathsf F'}$ cannot move any node  $\delta:g(Y)^{\OV{\phi(g(Y))}}$.
	
	\end{description}


We conclude then that, for all $Y\in \BV{\bb E'}$, $Y$ is $\phi(g(Y))$-eliminable.
It remains to check that for all $Y,Z\in \BV{\bb E'}$, $Y^{\phi(g(Y))}$ and $Z^{\phi(g(Y))}$ are coherent. It can be checked that for any parallel nodes $\alpha:Y^{\OV{\phi(g(Y))}}, \beta: Z^{\OV{\phi(g(Z))}}$ in $\bb E'$, $g(\alpha)$ and $g(\beta)$ are parallel in $\bb E$. Hence, if  $Y^{\phi(g(Y))}$ and $Z^{\phi(g(Y))}$  are not coherent, then $g(Y)^{\phi(Y)}$ and $g(Z)^{\phi(Z)}$ are not coherent, against the assumption.
%
%This leads to the following cases:
%
%	\begin{itemize}
%%	\item for all $i=1,\dots,k$, the terminal nodes $\beta_{i}:\mm\bullet$, which produce the conflicts $(\cc\bullet,  Y^{d})$, for all $\cc{T_{ij}}=Y^{\OV d}$;
%	\item if  $k=1$ and $\cc X$ does not occur in any of the $\cc{T_{1j}}$	, a conflict $(\mm\bullet, Z^{e})$, whenever in some of the sub-trees $\mm{U_{i}}$ of $\mathsf T$ there is some node $\delta:Z^{\OV e}$ which is parallel to some node $\eta: \mm X$.
%	\end{itemize}
%	
%Since $\psi(\bullet)=\cc{cyan}$, the only conflicts that $\psi$ can generate 	are of the form $(\cc\bullet,Y^{d})$, with $Y_{d}=\cc{T_{ij}}$, whenever $\psi(Y)=d$. However, in this case, since $(\cc X,Y^{d})$ is a conflict in $\mathsf T$, it must be $\psi(Y)=\phi(Y)=\OV d$. 
%
%\item[($\cc V\leadsto_{\mm X}\cc{V'}$)]
%
%
%\item[($\mm V\leadsto_{\cc X}\mm{V'}$)] This case is dual to the previous case, by switching $\cc{cyan}$ and $\mm{magenta}$.
%
%
%\item[($\mm V\leadsto_{\mm X}\mm{V'}$)] This case is dual to the first case, by switching $\cc{cyan}$ and $\mm{magenta}$.
\end{description}
\end{proof}







==> mubb.tex <==
% !TEX root = FSCDYonedaSubmission.tex




%By Proposition \ref{prop:yonered} any type $A$ of $\NYY$ is isomorphic to a type built from variables, high-school algebra operations and fixpoints. In this section we use this fact to show that $\NYY$ is equivalent to the smallest category endowed with such operations, the 
%
%\emph{free cartesian closed $\mu$-bicomplete category} $\mu\BB B$\cite{Santocanale2002, Basold2016}. 
%Similarly to $\NY$, we can prove Yoneda-equalities using $\varepsilon$-rules corresponding to a \emph{strong dinaturality} condition \cite{Uustalu2011}.  

% program equivalence in categories with a natural number objects \cite{okada}. 
%we show that the 
% a syntactic equivalence arising from a \emph{strong dinaturality} condition \cite{Uustalu2011}, we prove that program equivalence is undecidable in this fragment.


%Beyond $\NYY$, we will use the following type systems (all rules are recalled in App. \ref{appN}): the extension $\Ntot$ of $\Ndv$ with $\mu$ and $\nu$-types; the quantifier-free fragment $\NImu$ of $\Ntot$; the fragment $\Nmu$ obtained by restricting  the types of $\NYY$ to $\C P$ (Def. \ref{def:poly}).

The \emph{free cartesian closed $\mu$-bicomplete category} $\mu\BB B$ \cite{Santocanale2002,Basold2016} is $\CTX_{\beta\eta}^{0}(\NImu)$. 
We will make use in this section of the fragment $\Nmu$ of $\NYY$ in which the types correspond to pseudo-polynomials $\C P$ (Def. \ref{def:poly}). 







%Similarly to the case with $\kappa\leq 2$, the restriction of $\C E$ to $\C P$ yields a fragment $\Nmu$ of $\NY$, that we call the \emph{polynomial fragment}. 
%%The restriction of universal types to pseudo-polynomials yields a fragment $\NRP$ of $\NY$, that we call the \emph{finite polynomial fragment}. 
%%\begin{definition}
%%The \emph{polynomial fragment} $\Nmu$ is generated by the grammar
%%$$
%%A,B :=  X \mid A\To B\mid \forall X. \pp(X; \vec A) \mid \exists X. X\times (X\To \pp(X;\vec A))
%%$$
%%where $\pp(X;\vec X)$ is a quasi-polynomial. 
%%\end{definition}
%%\begin{corollary}
%
%
%The extension $\Ntot$ of $\Ndv$ with least and greatest fixpoints is standard and its syntax and $\beta\eta$-theory are recalled in App. \ref{appN}. %The 
%$\beta\eta$-theory of this system is also recalled in App. \ref{appN}.

%The polynomial translation $^{*}$ restricts to an embedding of $\Ntot$ into $\Nd$ (in fact, into $\NYY$), using Lemma \ref{lemma:pseudopp}.
%As in the case of $\BB B$, $^{*}$ scales to a functor $\mu\BB B\to \CTX_{\ctx}(\NYY)$ but \emph{not} into a functor
%$^{*}: \mu\BB B\to \CTX_{\beta\eta}(\NYY)$. Again, while $\beta$-rules are preserved, the non-local $\eta$-rules for $\mu,\nu$ are not preserved because Yoneda equalities are not isomorphisms under $\beta\eta$. 




%Again, such translations do not scale into functors between the respective $\beta\eta$-categories, since Yoneda equalities are not isomorphisms in these categories. Instead, Yoneda equalities can be seen to follow from non-local 

 $\varepsilon$-rules can be introduced for any universal type $\forall X.A$ of $\NYY$, corresponding to \emph{strong dinaturality} conditions \cite{Uustalu2011}.  Since these rules are rather involved to describe, we will limit here to consider some special case and we will rather exploit the remark below.


\begin{remark}\label{rem:unicity}
The correspondence between universal types in $\NYY$ and $\mu,\nu$-types provides a way to compute $\varepsilon$-equivalence in an indirect way. In fact, the $\varepsilon$-rules express an \emph{initiality}/\emph{finality} condition (essentially corresponding to the $\eta$-rules for such types, see App. \ref{appN}), which can be read  as the uniqueness of a function defined by an inductive/co-inductive principle. 
For example in the case of $\nat\simeq \mu X(X+1)$ the $\varepsilon$-rule is as in Fig. \ref{fig:nat}.
Let $C=\nat$, $u= \sss$, $D$  (the successor function) and $\rr{\TT C}$ be given by some function $f: \nat \To A$. Then the $\varepsilon$-rule yields the \emph{uniqueness rule} in Fig. \ref{fig:uniqnat}, which expresses the uniqueness of functions defined by iterations. 
We exploit this correspondence to establish the unidecidability of the equivalence generated by $\varepsilon$-rules (see \cite{LongVersion}, Thm. 6.10).

%
% expresses that whenever $f(\sss x)= v(f x)$ and $f(0)=a$, the function $f$ is equivalent to the function defined by iteration $g(x)\mapsto v^{x}(a)$. 
\end{remark}

The validity of Yoneda equalities under strong dinaturality condition yields:
\begin{lemma}[Yoneda lemma for $\kappa\leq 3$, \cite{Uustalu2011}]
Whenever $A,B\in \Pos_{X}$ and $C\in \Neg_{X}$,  $\forall X. (\forall Y.A\To X)\To B \equiv_{\varepsilon} B[\mu X.\exists Y.A/X]$ and $\forall X. (\forall Y.X\To A)\To C \equiv_{\varepsilon}C[\nu X.\forall Y.A/X]$.
\end{lemma}

%\end{remark}

% that of the type of \emph{recursive integers with one parameter}. % $\rrec=(\mu X.\forall Y.( \int\times Y\times X)+  1  )^{*}$. 

%
%
%\begin{remark}
%By Prop. \ref{prop:yonered} we can suppose w.l.o.g.  that a type $\forall X.A$ with $\kappa_{X}(A)\leq 3$ is either of the form
%$\forall X\forall \vec Y. A_{1}\To \dots \To A_{k}\To A_{k+1}$, where $A_{i}= P_{i}\To X$, with $P_{i}\in \Pos_{X}$ for $i=1, \dots, k$ and $A_{k+1}\in \Pos_{X}$, or of the form
%$\forall X\forall \vec Y.  A_{1}\To \dots \To A_{k}\To A_{k+1}$, where $A_{i}= X\To P_{i}$ with $P_{i}\in \Pos_{X}$ for $i=1,\dots, k$ and $A_{k+1}\in \Neg_{X}$.
%\end{remark}
%
%
%\begin{definition}[$\varepsilon$-theory for $\kappa\leq 3$]
%The \emph{positive $\varepsilon$-rule} is the rule in Fig. \ref{fig:supereps1}, where $A=\forall \vec Y. A_{1}\To \dots \To A_{k}\To A_{k+1}$, where $A_{1},\dots, A_{k+1}\in \Pos_{X}$.  
%The \emph{negative $\varepsilon$-rule} is defined dually
%% rule in Fig. \ref{fig:supereps2}, where
%for  $A=\forall \vec Y. A_{1}\To \dots \To A_{k}\To A_{k+1}$, where $A_{1},\dots, A_{k+1}\in \Neg_{X}$.  
%
%
%We let $\simeq_{\varepsilon}$ be the smallest theory of $\Nd^{\kappa\leq 3}$ generated by $\beta$, $\eta$ and $\varepsilon$-rules.
%\end{definition}
%
%\begin{figure}
%\adjustbox{scale=0.75, center}
%{$
%\AXC{$\left( \Gamma\vdash u_{i}: A_{i}[C/X]\To C  \right )_{i=1,\dots,k}$} 
%\AXC{$\left( \Gamma\vdash v_{i}: A_{i}[D/X]\To D  \right )_{i=1,\dots,k}$} 
%\AXC{$\rr{\TT C}: C\vdash^{\Gamma} D$}
%\AXC{$\left (\rr{\TT C}[ u_{i}[\ ]] \simeq v_{i}\Fun{X}{A_{i}}(\rr{\TT C}) : A_{i}[C/X]\vdash^{\Gamma}D\right )_{i=1,\dots,k}$}
%\QuaternaryInfC{$
%\Gamma, x: A\vdash \Fun{X}{A_{k+1}}(\rr{\TT C})[ xCu_{1}\dots u_{k}] \simeq xD v_{1}\dots v_{k} : A_{k+1}[D/X]
% $}
%\DP
%$}
%\caption{Positive $\varepsilon$-rule for $\kappa=3$.}
%\label{fig:supereps1}
%\end{figure}
%%\begin{figure}
%\adjustbox{scale=0.75, center}
%{$
%\AXC{$\left( \Gamma\vdash u_{i}: A_{i}[D/X]\To D  \right )_{i=1,\dots,k}$} 
%\AXC{$\left( \Gamma\vdash v_{i}: A_{i}[C/X]\To C  \right )_{i=1,\dots,k}$} 
%\AXC{$\rr{\TT C}: D\vdash^{\Gamma} C$}
%\AXC{$\left (\rr{\TT C}[ u_{i}[\ ]] \simeq v_{i}\Fun{X}{A_{i}}(\rr{\TT C}) : A_{i}[D/X]\vdash^{\Gamma}C\right )_{i=1,\dots,k}$}
%\QuaternaryInfC{$
%\Gamma, x: A\vdash \Fun{X}{A_{k+1}}(\rr{\TT C})[ xDu_{1}\dots u_{k}] \simeq xC v_{1}\dots v_{k} : A_{k+1}[C/X]
% $}
%\DP
%$}
%\caption{Negative $\varepsilon$-rule for $\kappa=3$.}
%\label{fig:supereps2}
%\end{figure}

%
%Instead of describing this (rather complex) theory in detail, we will just a describe $\varepsilon$-rules expressing the strong dinaturality conditions for two specific types, that will suffice to our discussion: the type of integers $\nat$ (see Fig. \ref{fig:nat}) and the type of \emph{recursors with parameters in $Y$} $\REC=\forall X. (\nat\To Y \To X\To X)\To (Y\To  X) \To Y\To \nat \To X$ (see Fig: \ref{fig:rec}).


%\begin{definition}[strong dinaturality]
%Let $F,G:\BB C^{op}\times \BB C\to \BB D$ be functors. A \emph{strong dinatural transformation} from $F$ to $G$ is a family $\theta_{a}\in \BB D(F(a,a),G(a,a))$ such that for all $a,b$, $f\in \BB C(a,b)$, given $g,h$ making $(*)$ commute, the outer diagram commutes. 
%
%\adjustbox{scale=0.7, center}{
%$
%\begin{tikzcd}
%   &    F(a,a) \ar{rr}{\theta_{a}} \ar{rd}{F(a,f)}  & & G(a,a) \ar{rd}{G(a,f)} &  \\ 
%c \ar{ru}{g} \ar{rd}{h} &  (*)& F(a,b) & & G(a,b) \\
%  & F(b,b) \ar{rr}[below]{\theta_{b}} \ar{ru}[right]{F(f,b)} & & G(b,b) \ar{ru}[right]{G(f,b)} & 
%\end{tikzcd}
%$}
%
%\end{definition}

%\begin{figure}
%
%\caption{Strong dinaturality}
%\label{fig:pare}
%\end{figure}


%It is not difficult to extend Def. \ref{} to show that \emph{any} type $A$ of $\Nd$ yields for all variable $X$ a functor $\Fun{X}{A}: \CTX_{\beta\eta}(\Nd)^{\mathsf{op}}\times \CTX_{\beta\eta}(\Nd) \to \CTX_{\beta\eta}(\Nd)$. From the definition above we can then compute $\varepsilon$-rules for all type $\forall X.A$ in $\NYY$.





\begin{figure}[t]
\begin{subfigure}{\textwidth}
\adjustbox{scale=0.8, center}
{$
\AXC{$ \Gamma\vdash u: C\To C  $} 
\AXC{$ \Gamma\vdash v: D\To D $}
\AXC{$\rr{\TT C}: C\vdash^{\Gamma} D$}
\AXC{$\rr{\TT C}[ u[\ ]] \simeq v\rr{\TT C} : C\vdash^{\Gamma}D$}
\QuaternaryInfC{$
\Gamma, x:\nat, y:C\vdash \rr{\TT C}[ xCuy] \simeq xD v\rr{\TT C}[y] : D
 $}
\DP
$}
\caption{$\varepsilon$-rule for $\nat$.}
\label{fig:nat}
\end{subfigure}
\begin{subfigure}{\textwidth}
\adjustbox{scale=0.8, center}{
$
\AXC{$\Gamma\vdash f: \nat \To D $}
\AXC{$\Gamma\vdash v: D \To D$}
\AXC{$\Gamma, x:\nat\vdash f(\sss x) \simeq_{\varepsilon} v(fx):D$}
\TrinaryInfC{$ \Gamma,x:\nat \vdash fx \simeq_{\varepsilon} xD v (f\mathsf 0):D$}
\DP 
$}
\caption{Uniqueness rule for $\nat$.}
\label{fig:uniqnat}
\end{subfigure}
\caption{The $\varepsilon$-rules for $\nat$ yields a unicity condition for iteratively-defined functions.}
\end{figure}

%Using $\varepsilon$-rules and arguing similarly to Lemma \ref{lemma:yozz} we can prove:


Similarly to the case of $\NY$, the maps $^{\sharp}:\C E_{3}\to \C P$, $^{*}:\mu\C H\to \C P$ and $^{\flat}: \C E_{3}\to \mu \C H_{0}$ yield functors $^{\sharp}: \CTX_{\varepsilon}(\NYY) \to \CTX_{\varepsilon}(\Nmu)$, $^{*}: \CTX_{\varepsilon}(\Ntot)\To \CTX_{\varepsilon}(\Nmu)$ and $^{\flat}: \CTX_{\varepsilon}(\NYY) \to \CTX_{\beta\eta}(\mu \BB B)$. 



%From this we deduce that we have functors $^{\sharp}: \CTX_{\varepsilon}(\NYY) \to \CTX_{\varepsilon}(\Nmu)$, $^{*}: \mu \BB B\to \CTX_{\varepsilon}(\Nmu)$ and $^{\flat}: \CTX_{\varepsilon}(\NYY) \to \mu\BB B$. 
%We provide a sketch of how these functors yield equivalences between the respective categories.

\begin{theorem}
%\begin{itemize}
%\item 
$\CTX_{\varepsilon}^{0}(\NYY) \cong \CTX_{\varepsilon}^{0}(\Nmu)    \cong  \mu \BB B$.
%\end{itemize}
\end{theorem}
\begin{proof}[Proof (sketch)]
%To prove the equivalence between $\CTX_{\varepsilon}^{0}(\NYY)$ and $\mu \BB B$ 
We establish the chain of equivalences:
$$
\CTX_{\varepsilon}^{0}(\NYY) 
\ \stackrel{(*)}{\cong}
\ \CTX_{\varepsilon}^{0}(\Nmu) 
 \ \stackrel{(**)}{  \cong}  \  
\CTX_{\varepsilon}^{0}(\Nd^{\mu\mathsf{Poly}}_{0,1,+,\times}) \ \stackrel{(***)}{\cong } \ 
\mu\BB B 
$$
 $(*)$ is obtained as in Theorem \ref{thm:equiva} (iii.) using a generalization of Lemma \ref{thm:appa} (2) with $\NYY$ and $\Nmu$ instead of $\NY$ and $\NRP$ (see \cite{LongVersion}, Prop. A.1). 
Equivalence $(**)$ follows from Theorem \ref{thm:equiva} by arguing as in Remark \ref{rem:equiva}.
Finally, equivalence $(***)$ follows from the remark that the restrictions of $^{*}$ and $^{\flat}$ yield inverse maps between the types of $\Nd^{\mu\mathsf{Poly}}_{0,1,+,\times}$ and those of $\mu\BB B$, considered up to $\simeq_{0}$. 
A routine inductive argument shows then that the mappings $t\mapsto t^{*}$ and $u\mapsto u^{\sharp}$ are inverse each-other (modulo $\varepsilon$). %proving that $\CTX_{\varepsilon}^{0}(\Nd^{\mu\mathsf{Poly}}_{0,1,+,\times}) $ and 
%$\mu \BB B$ are isomorphic categories. 
\end{proof}

%
%Contextual equivalence in $\mu\BB B$ is undecidable \cite{Basold2016}. However, at the present state we know of no coherence result (i.e. $\simeq_{\ctx}=\simeq_{\beta\eta}$) for this theory. In App \ref{app??} we provide a direct argument showing that $\varepsilon$-equivalence is undecidable in $\NYY$. This implies in particular the undecidability of $\simeq_{\beta\eta}$ in $\mu\BB B$, using a result from \cite{Okada1999}. 


%To prove  the equivalence of $ \CTX_{\varepsilon}^{0}(\Nd^{\kappa\leq 3}_{0,1,+,\times})  $ and  $\CTX_{\varepsilon}^{0}(\Nd^{\mu\mathsf{Poly}}_{0,1,+,\times})$, we first construct a surjective map from the types of the first to those of the second using Lemma \ref{lemma:fixp}.
%
%\begin{lemma}
%There exists a surjective map $^{\sharp}: \Nd^{\kappa\leq 3}_{0,1,+,\times} \to  \Nd^{\mu\mathsf{Poly}}_{0,1,+,\times}$
%such that for all $e$ in $\Nd^{\kappa\leq 3}_{0,1,+,\times}$ there exists an isomorphism $u_{e}:e\to e^{\sharp}$ in 
%$\CTX_{\varepsilon}^{0}(\Nd^{\kappa\leq 3}_{0,1,+,\times})$.
%\end{lemma}
%\begin{proof}
%Let $\mathsf W$ be a new countable set of variables. For any $e$ type of $\Nd^{\kappa\leq 3}_{0,1,+,\times}$ we let $e^{\mathsf W}$ be obtained by replacing each occurrences of $0,1,+,\times$ by its associated pseudo-polynomial $\int_{W}\pp(W ; \vec e)$  in $\Nd$ \emph{with the bound variable $W$ chosen in $\mathsf W$}. By Lemma \ref{lemma:piu}, $\kappa_{X}(e^{\mathsf W})=\kappa_{X}(e)$, whence we can now translate the $e^{\mathsf W}$ into $\Nmu$ using Lemma \ref{lemma:fixp}. We finally obtain a type $e^{\sharp}$ in $\Nd^{\mu\mathsf{Poly}}_{0,1,+,\times}$ by \emph{translating back} all $\int_{W}\pp(W; \vec e)$, with $W\in \mathsf W$, into $\pp^{\sharp}(\vec e)$. 
%\end{proof}
%
%
%To apply Lemma \ref{lemma:fullsub} it remains to show that $\CTX_{\varepsilon}^{0}(\Nd^{\mu\mathsf{Poly}}_{0,1,+,\times})$ is a full subcategory of $\CTX_{\varepsilon}^{0}(\Nd^{\kappa\leq 3}_{0,1,+,\times})$. This fact is just the extension of Lemma \ref{thm:appa} to $\kappa=3$, i.e. to the translation of initial algebras/final coalgebras, and can be checked similarly by using the $\varepsilon$-rules for $\kappa=3$. 
%
%\begin{proposition}\label{prop:euno}
%$\CTX_{\varepsilon}^{0}(\Nd^{\kappa\leq 3}_{0,1,+,\times}) $ is equivalent to  
%$\CTX_{\varepsilon}^{0}(\Nd^{\mu\mathsf{Poly}}_{0,1,+,\times})$.
%\end{proposition}
%




%
%\begin{figure}[t]
%\adjustbox{scale=0.8, center}
%{$
%\AXC{$ \Gamma\vdash u: \nat \To Y \To A\To A  $} 
%\AXC{$ \Gamma\vdash v: \nat \To Y \To  B\To B $}
%\AXC{$\rr{\TT C}: A\vdash^{\Gamma} B$}
%\AXC{$\rr{\TT C}[ uyz[\ ]] \simeq vyz\rr{\TT C} : A\vdash^{\Gamma, y:\nat, z:Y}B$}
%\QuaternaryInfC{$
%\Gamma, x:\REC,y:\nat, z:Y, w:A\vdash \rr{\TT C}[ xAuyzw] \simeq xB v yz\rr{\TT C}[w] : B
% $}
%\DP
%$}
%\caption{$\varepsilon$-rule for $\REC$.}
%\label{fig:rec}
%\end{figure}
%%
%
%
%\begin{definition}
%Let $F:\BB C\to \BB C$ be a functor. An \emph{  s a pair $(A,\rr{\mathsf C})$, where 
%$\rr{\mathsf C}: T[A/X]\to A$. A \emph{$T$-algebra morphism from $(A,\rr{\mathsf C})$ to $(B,\rr{\mathsf D})$} is a context
%$\rr{\mathsf E}: A\vdash B$ such that 
%$$
%  \rr{ \mathsf E} \circ \rr{\mathsf C }\simeq_{\varepsilon} \rr{\mathsf D}\circ \Fun{X}{T}(\rr{\mathsf E})
%$$
%\end{definition}

%
%\begin{definition}
%An \emph{initial algebra} for $T$ is a $T$-algebra $(\mu X.T, \mathsf{in}_{T})$ such that for all $T$-algebra $(A,t)$ there exists a unique $T$-algebra morphism $\mathsf{fold}_{T}(t): \mu X.T \to A$.
%
%\end{definition}

%\begin{proof}
%The equation  with $0$ is easily computed. Fo
%


%Using Yoneda equalities it is not difficult to show that
%$\int_{X} X^{(\nat \times Y \times X^{Y}\times X^{\nat \times Y\times X})} \simeq  (\mu  X ((\nat \times Y\times X)+Y))\times \nat \times Y$. In fact using the $\varepsilon$-rules we can prove:
%
%\begin{lemma}\label{lemma:muxxi}
%$\nat \equiv_{\varepsilon}\mu X.X+1$, $\REC \equiv_{\varepsilon} (\mu X. (\nat \times Y\times X)+Y)\times \nat \times Y$.
%
%\end{lemma}
%	
%	
%	A simple consequence of Lemma \ref{lemma:muxxi} is the following:
%\begin{lemma}\label{lemma:predecessor}
%\begin{itemize}
%\item $x:\nat  \vdash x \simeq_{\varepsilon} x\nat \mathsf S \mathsf 0$.
%\item $\mathsf P \mathsf S x\simeq_{\varepsilon}x$.
%\end{itemize}
%\end{lemma}
%\begin{proof}
%TODO.
%\end{proof}
%	
%
%%Following \cite{pare} we define strong dinatural transformations 
%
%The reason for considering the type $\REC$ is that we wish to exploit the following result
%
%
%\begin{theorem}[Okada, Scott]\label{th:okada}
%Let $S$ be a system containing the type $\nat$ of integers (with terms $\zz:\nat$ and  $\sss:\nat\To \nat$), closed by arrow types and having, for all type $A,B$ a recursor $\rec_{A,B}: (\nat \To A\To B\To B)\To (A\To B)\To (A\To \nat\To B)$ satisfying
%$$
%\rec_{A,B} h u a \zz= ua \qquad 
%\rec_{A,B}h u a (\sss x)= h x a (\rec_{A,B} h u a x)
%$$
%Let $\simeq_{\gamma}$ be an equivalence over $S$ containing $\simeq_{\beta},\simeq_{\eta}$ and closed by  the following rule:
%$$
%\AXC{$f x(\mathsf S y) \simeq h xy(fxy)$}
%\RL{($\mathsf U_{A,B,f}$)}
%\UIC{$f \simeq \rec_{A,B} h  (\lambda x.fx0)  $}
%\DP
%$$
%Then $\simeq_{\gamma}$ is undecidable.
%\end{theorem}
%
%
%In fact, using Lemma \ref{lemma:predecessor}, it can be easily checked that: 
%\begin{lemma}\label{lemma:recursor}
%The term $\rec: \forall XY. (\nat\To Y \To X\To X)\To (Y\To  X) \To Y\To \nat \To X$ given by
%$\rec  X Y h x a y = y X   \lambda z. h (\mathsf{P}y) a z \   (xa)  $
%is a recursor in $\Nd_{\kappa\leq 3}$ under $\simeq_{\varepsilon}$.
%\end{lemma}
%	
%r the other equation we have
%%$\rec XY hx a(\mathsf Sy)\simeq_{\beta}
%%h(\mathsf P \mathsf Sy)a  ( y X \lambda z.h(\mathsf Py)az) (xa)) \simeq_{\beta}
%%h (\mathsf P\mathsf Sy) a(\rec XY hx ay)$, so the claim follows from Lemma \ref{lemma:predecessor}.
%%
%%\end{proof}
%
%We can show that the rule  $(\mathsf U_{A,B,f})$ follows from the $\varepsilon$-rules:
%\begin{theorem}
%%The rule $(\mathsf U_{A,B,f})$ holds in $\Nd_{\kappa\leq 3}$ under $\simeq_{\varepsilon}$ with $\rec$ as recursor.
%$\simeq_{\varepsilon}$, and \emph{a fortiori} $\simeq_{\ctx}$, are undecidable in $\NYY$.
%
%\end{theorem}
%\begin{proof}
%Let $\mathsf Z: \nat \To A \To \nat \To \nat$ be the term $\mathsf Z xyz= \mathsf Sz$. We claim that 
%$\rec A \nat \mathsf  Z \lambda x.0  a y \simeq_{\varepsilon} y$.  In fact
%$\rec A \nat \mathsf  Z \lambda x.0  a y \simeq_{\beta}
%y \nat \lambda z. \mathsf Z (\mathsf Py) a z \mathsf 0 \simeq_{\beta\eta} y \nat \mathsf S \mathsf 0\simeq_{\varepsilon}y$, by Lemma \ref{lemma:predecessor}.
%Let now $f: A\To \nat \To B$. If $ f a( \mathsf Z x ay)  \simeq_{\varepsilon} h x a (f ax)$, we deduce, by the $\varepsilon$-rule in Fig. \ref{fig:rec} with $\rr{\TT C}= fa[\ ]: \nat \vdash B$, that $
%f a (\rec A \nat \mathsf Z \lambda  x.0 a y) \simeq_{\varepsilon}
%\rec A B h  \lambda x. fa0  \ ay
%$. By what we just proved this implication corresponds exactly to $(U_{A,B,f})$.
%The claim follows then from Theorem \ref{th:okada} and Lemma \ref{lemma:recursor}.
%\end{proof}
%
%%\begin{theorem}
%%\end{theorem}
%%\begin{figure}
%%\adjustbox{scale=0.7,center}{
%%\begin{tikzcd}
%%\nat \to A\to \nat \to \nat  \ar{rd}    \ar{rrr}{\rec A \nat} & & &    \nat\to A \to \nat \to \nat  \ar{rd}   &  \\
%%   &   \nat \to A \to \nat \to B  & & & \nat \to A \to \nat \to B \\
%%\nat \to A \to B  \to B \ar{ru} \ar{rrr}[below]{\rec A B} & & &  B\to A \to \nat \to B \ar{ru}
%%\end{tikzcd}
%%}
%%\caption{Strong dinaturality for the type of $\rec$}
%%\label{fig:sdinrec}
%%\end{figure}
%%
%%
%%
%%














==> undecidability.tex <==




% !TEX root = YonedaTryAgain.tex





Using the argument from Section 7, to establish that the $\varepsilon$-theory and contextual equivalence coincide and are equivalent for $\NY$, we only need to prove the following:

\contextual*
\begin{proof}%[Proof of Prop. \ref{prop:equivalents}.]
\begin{description}
\item[(i.$\To$ ii.)] Since $\simeq_{\ctx}$ is the maximal consistent theory, it is clear that $\simeq_{\varepsilon}\subseteq \simeq_{\ctx}$.



\item[(ii.$\To$ iii.)] 

Suppose $\Gamma^{\flat}\vdash_{\NI} t^{\natural}\not\simeq_{\beta\eta}u^{\natural}:A^{\natural}$. Since $\simeq_{\beta\eta}$ and $\simeq_{\ctx}$ coincide in $\NI$, there exists a context $\TT C: (\Gamma^{\flat}\vdash A^{\flat})\To (\vdash 1+1)$ such that $\TT C[t^{\natural}]\not\simeq_{\beta\eta}\TT C[u^{\natural}]$. Observe that this also implies $\TT d_{B}^{-1}[\TT C[t^{\natural}]]\not\simeq_{\beta\eta}\TT d_{B}^{-1}[\TT C[u^{\natural}]]$, where $B=\forall X.X\To X \To X$.

Let $\TT F: (\Gamma\vdash A)\to (\Gamma^{\flat}\vdash A^{\flat})$ be 
$(\lambda x_{1}.\dots. \lambda x_{k}. \TT d_{B}^{-1}[ x ])\TT d_{A_{1}}^{-1}[x_{1}]\dots \TT d_{A_{k}}^{-1}[x_{k}]$, where $\Gamma=\{x_{1}:A_{1},\dots, x_{k}:A_{k}\}$. Then $\TT F[t]\simeq_{\beta\eta}t^{\natural}$ and $\TT F[u]\simeq_{\beta\eta}u^{\natural}$. 


Let now $\TT E:(\Gamma\vdash_{\Ndv} A)\to (\vdash_{\Ndv}\forall X.X\To X\To X)$ be the context $\TT d_{B}^{-1}\circ\TT C\circ\TT F$, so that $\TT E^{\sharp}:(\Gamma\vdash_{\NY} A)\to (\vdash_{\NY}\forall X.X\To X\To X)$. We also have $\TT E\simeq_{\varepsilon}\TT E^{\sharp}$ by Th. \ref{thm:full}. We now have
$\TT E^{\sharp}[t] \simeq_{\varepsilon} \TT E[t] \simeq_{\beta\eta} \TT d_{B}^{-1}[ \TT C[t^{\natural}]] \not\simeq_{\beta\eta}
\TT d_{B}^{-1}[\TT C[u^{\natural}]] \simeq_{\beta\eta} \TT E[u]\simeq_{\varepsilon}\TT E^{\sharp}[t]$, so we can conclude that 
$t \not \simeq_{\ctx} u$.


\item[(iii.$\To$ i.)] This immediately follows from the fact $t^{\natural},u^{\natural}$ are obtained from $t,u$ by applying isomorphisms relative to $\varepsilon$-equivalence.
\end{description}
\end{proof}



\begin{figure}[t]
\begin{subfigure}{\textwidth}
\adjustbox{scale=0.8, center}
{$
\AXC{$ \Gamma\vdash u: C\To C  $} 
\AXC{$ \Gamma\vdash v: D\To D $}
\AXC{$t[x]: C\vdash^{\Gamma} D$}
\AXC{$t[ ux] \simeq v\rr{\TT c} : C\vdash^{\Gamma}D$}
\QuaternaryInfC{$
\Gamma, z:\nat, y:C\vdash t[ zCuy] \simeq zD vt[y] : D
 $}
\DP
$}
\caption{$\varepsilon$-rule for $\nat$.}
\label{fig:nat}
\end{subfigure}
\begin{subfigure}{\textwidth}
\adjustbox{scale=0.8, center}{
$
\AXC{$\Gamma\vdash f: \nat \To D $}
\AXC{$\Gamma\vdash v: D \To D$}
\AXC{$\Gamma, x:\nat\vdash f(\sss x) \simeq_{\varepsilon} v(fx):D$}
\TrinaryInfC{$ \Gamma,x:\nat \vdash fx \simeq_{\varepsilon} xD v (f\mathsf 0):D$}
\DP 
$}
\caption{Uniqueness rule for $\nat$.}
\label{fig:uniqnat}
\end{subfigure}
\caption{The $\varepsilon$-rules for $\nat$ yields a unicity condition for iteratively-defined functions.}
\end{figure}

%
\begin{figure}[t]
\adjustbox{scale=0.8, center}
{$
\AXC{$ \Gamma\vdash u: \nat \To Y \To A\To A  $} 
\AXC{$ \Gamma\vdash v: \nat \To Y \To  B\To B $}
\AXC{$\rr{t}[x]: A\vdash^{\Gamma} B$}
\AXC{$\rr{t}[ uyzx] \simeq vyz\rr{t} : A\vdash^{\Gamma, y:\nat, z:Y}B$}
\QuaternaryInfC{$
\Gamma, x:\REC,y:\nat, z:Y, w:A\vdash {t}[ xAuyzw] \simeq xB v yz {t}[w] : B
 $}
\DP
$}
\caption{$\varepsilon$-rule for $\REC$.}
\label{fig:rec}
\end{figure}
%


We now turn to the problem of showing the undecidability of the $\varepsilon$-theory in $\NYY$.
The correspondence between universal types in $\NYY$ and $\mu,\nu$-types provides a way to compute $\varepsilon$-equivalence in an indirect way. In fact, the $\varepsilon$-rule for a type $\forall X.A$ of $\NYY$ can be interpreted as a principle expressing the \emph{uniqueness} of a function defined by an inductive/co-inductive principle. 
For example, in the case of the type $\nat=\forall X.(\cc X\To \mm X)\To (\mm X\To \cc X)$, from the isomorphism
$\nat\equiv_{\cc X} \mu X(X+1)$ we deduce the validity of the  $\varepsilon$-rule in Fig. \ref{fig:nat}.
Let $C=\nat$, $u= \sss$, $D$  (the successor function) and $\rr{\TT c}$ be given by some function $f: \nat \To A$. Then the $\varepsilon$-rule yields the \emph{uniqueness rule} in Fig. \ref{fig:uniqnat}, which expresses the uniqueness of functions defined by iterations. 


We will exploit this correspondence to establish the undecidability of the equivalence generated by $\varepsilon$-rules from the result below.



\begin{theorem}[Okada, Scott]\label{th:okada}
Let $\mathsf S$ be a system containing the type $\nat$ of integers (with terms $\zz:\nat$ and  $\sss:\nat\To \nat$), closed by arrow types and having, for all type $A,B$ a recursor $\rec_{A,B}: (\nat \To A\To B\To B)\To (A\To B)\To (A\To \nat\To B)$ satisfying
\begin{equation}
\rec_{A,B} h u a \zz= ua \qquad 
\rec_{A,B}h u a (\sss x)= h x a (\rec_{A,B} h u a x)
\end{equation}
Let $\simeq_{\gamma}$ be an equivalence over $\mathsf S$ containing $\simeq_{\beta},\simeq_{\eta}$ and closed by  the following rule:
\begin{equation}\label{ruleU}
\AXC{$f x(\mathsf S y) \simeq h xy(fxy)$}
%\RL{($\mathsf U_{A,B,f}$)}
\UIC{$f \simeq \rec_{A,B} h  (\lambda x.fx0)  $}
\DP \tag{U}
\end{equation}
for all $f: A\To \nat\To B$ and $h: \nat\To A\To B\To B$.
Then $\simeq_{\gamma}$ is undecidable.
\end{theorem}

Let us first show that we can restrict to a weaker rule:


\begin{lemma}\label{lemma:UUU}
The rule \eqref{ruleU} is deducible from the rule
\begin{equation}\label{wU}
\AXC{$f x(\mathsf S y) \simeq h yx(fxy)$}
%\RL{($\mathsf U_{A,B,f}$)}
\UIC{$f ay \simeq \rec_{A,B} h  (\lambda x.fa0) ay $}
\DP\tag{wU}
\end{equation}

\end{lemma}
\begin{proof}
Let $Q = \rec_{A,B}h(\lambda x.fx\mathsf 0) $. Since 
$Q a (\mathsf Sy) \simeq
h ya( Q a y)$  and $Qa\mathsf 0\simeq fa\mathsf 0$,  by \eqref{wU} we deduce
$Q a y \simeq \rec_{A,B}h(\lambda x.Qa0) a y \simeq
\rec_{A,B}h(\lambda x.fa\mathsf 0)ay$. 

Now, if $f x(\mathsf S y) \simeq h xy(fxy)$ holds, by \eqref{wU} we deduce 
$fay\simeq \rec_{A,B}h(\lambda x.fa0) a y $ and by composing this with the equivalence above we finally get 
$fay \simeq \rec_{A,B}h(\lambda x.fx0) a y$. 
\end{proof}




We now establish some preliminary properties of $\varepsilon$-equivalence over the type $\nat$. For simplicity, we  will work in 
an extension of $\NYY$ with product types.
We let $\mathsf 0=\Lambda X.\lambda fx.x$ and $\mathsf  s= \lambda y. \Lambda X.\lambda fx.f(yXfx)$, $\mathsf P=\lambda x. \pi_{2}\left ( x (\nat\times \nat) \lambda y.\langle \sss (\pi_{1}y), \pi_{1}y\rangle \langle \zz, \zz \rangle\right)$. 



\begin{lemma}\label{lemma:predecessor}
\begin{itemize}
\item $x:\nat  \vdash x \simeq_{\varepsilon} x(\nat)  ( \sss )  \mathsf 0$.
\item $\mathsf P( \sss x)\simeq_{\varepsilon}x$.
\end{itemize}
\end{lemma}
\begin{proof}
We prove both results as a consequence of unicity of iteration. If $Fx=x$, then $F\zz\simeq_{\beta}\zz (\nat)( \sss) \zz$ and $F(\sss x)= \sss x= \sss (Fx)$, whence by unicity $x=Fx\simeq_{\varepsilon} x (\nat )(\sss) \zz$. 

Let $\rr{\TT c}[x]:=x (\nat\times \nat) \lambda y.\langle \sss (\pi_{1}y), \pi_{1}y\rangle \langle \zz, \zz \rangle$.
We have $\mathsf P(\sss \zz)=\zz$ and, since $\mathsf P(\sss x)\simeq_{\beta} \pi_{1}\rr{\TT c}[x]$,
and $\pi_{1}\rr{\TT c}[\sss x]\simeq_{\beta} \sss (\pi_{1}\rr{\TT c}[x])$, we have 
 $\mathsf P(\sss(\sss x))\simeq_{\beta} \sss (\pi_{1} \rr{\TT c}[x])
\simeq_{\beta}\sss (\mathsf P(\sss x))$, so by unicity we conclude
$\mathsf P(\sss x)\simeq_{\varepsilon} x (\nat)( \sss) \zz \simeq_{\varepsilon}x$. 
\end{proof}
	
To apply Theorem \ref{th:okada} we will exploit the type $\REC=\forall X. (\nat\To Y \To X\To X)\To (Y\To  X) \To Y\To \nat \To X$. Observe that $\REC$ is isomorphic to the non-polymorphic type $(\mu X. (\nat \times Y\times X)+Y)\times \nat \times Y$. 
%, and its $\varepsilon$-rule is described in Fig. \ref{fig:rec}.
 Using Lemma \ref{lemma:predecessor}, it can be checked by induction that  the term $\rec: \forall Y.\REC$ given by
$\rec  (X)( Y) h x a y = y (X)(   \lambda z. h (\mathsf{P}y)a z)    (xa)  $
yields, for all types $A,B$ of $\NYY$, a recursor $\rec (A)(B)$ in $\Nd_{\kappa\leq 3}$ under $\simeq_{\varepsilon}$.

%We now show that the initiality condition  for $\REC$ (the $\varepsilon$-rule in Fig. \ref{fig:rec}) implies the rule  $(\mathsf U_{A,B,f})$:


%Using Yoneda equalities it is not difficult to show that
%$\int_{X} X^{(\nat \times Y \times X^{Y}\times X^{\nat \times Y\times X})} \simeq  (\mu  X ((\nat \times Y\times X)+Y))\times \nat \times Y$. In fact using the $\varepsilon$-rules we can prove:
%
%\begin{lemma}\label{lemma:muxxi}
%$\nat \equiv_{\varepsilon}\mu X.X+1$, $\REC \equiv_{\varepsilon} (\mu X. (\nat \times Y\times X)+Y)\times \nat \times Y$.
%
%\end{lemma}
	
%%Following \cite{pare} we define strong dinatural transformations 
%
%\begin{lemma}\label{lemma:recursor}
%For all type $A,B$ of $\NYY$ $\rec AB$ is a recursor in $\Nd_{\kappa\leq 3}$ under $\simeq_{\varepsilon}$.
%\end{lemma}
	

%Using the $\varepsilon$-rule for $\REC$ (Fig: \ref{fig:rec}) 

\begin{proposition}
The rule \eqref{ruleU} holds in $\NYY$ under $\simeq_{\varepsilon}$ with $\rec$ as recursor.

\end{proposition}
\begin{proof}
Let $\mathsf Z: \nat \To A \To \nat \To \nat$ be the term $\mathsf Z xyz= \mathsf sz$. We claim that 
$\rec(A)( \nat)( \mathsf  Z )(\lambda x.0 ) a y \simeq_{\varepsilon} y$.  In fact
$\rec (A) (\nat )(\mathsf  Z )(\lambda x.0 ) a y \simeq_{\beta}
y (\nat)( \lambda z. \mathsf Z (\mathsf Py) a z) \mathsf 0 \simeq_{\beta\eta} y( \nat)( \mathsf s) \mathsf 0\simeq_{\varepsilon}y$, by Lemma \ref{lemma:predecessor}.
Let now $f: A\To \nat \To B$. If $ f a( \mathsf Z x ay)  \simeq_{\varepsilon} h x a (f ax)$, we deduce, by the $\varepsilon$-rule in Fig. \ref{fig:rec} with $t[x]= fax: \nat \vdash B$, that $
f a (\rec (A)( \nat)( \mathsf Z)( \lambda  x.0 )a y) \simeq_{\varepsilon}
\rec (A)( B)( h)(  \lambda x. fa0)  \ ay
$. By what we just proved this implication corresponds to the rule \eqref{wU}, so we can conclude by Lemma \ref{lemma:UUU}.
%The claim follows then from Theorem \ref{th:okada}.
\end{proof}

\begin{corollary}
The $\varepsilon$-theory is undecidable in $\NYY$.

\end{corollary}
